Technical Design Report for PANDA Electromagnetic Calorimeter (EMC)

This document presents the technical layout and the envisaged performance of the Electromagnetic Calorimeter (EMC) for the PANDA target spectrometer. The EMC has been designed to meet the physics goals of the PANDA experiment, which is being developed for the Facility for Antiproton and Ion Research (FAIR) at Darmstadt, Germany. The performance figures are based on extensive prototype tests and radiation hardness studies. The document shows that the EMC is ready for construction up to the front-end electronics interface.

==> emc_main_costs.tex <==
\subsection{Cost Estimate}
%
At the present stage it is impossible to give a firm estimate of the
expected costs for the necessary investments, since there are diverse
options and open questions concerning the calorimeter components, which
rely on further research and development as well as on the results from
full size prototype studies. As a consequence, the required external and
internal amount of labour can not be judged at all. Only for some specific
components or materials an estimate can be given based on the present
general knowledge but not yet adapted to the specific needs of \Panda.

The mechanical support structure, thermal insulation and cooling system
can only be estimated based on similar detector set-ups such as \INST{CMS} ECAL.
There are large discrepancies of the costs for the mechanical housing of
crystal modules, depending on the selected material (fiber glass, carbon,
\etc) and the resulting manufacturing processes, which have severe impact
on the amount of labour. The proposed support structures and the
implementation into the magnet will be straightforward. However, details
on insulation and cooling technique can only be deduced from a full size
prototype of one completely filled slice of the barrel section. 

The dominating part of the overall costs of the calorimeter is determined
by the scintillator material and the photo sensor. The target calorimeter
comprises in the proposed geometry 19,030 crystals of $200\,\mm$ length
accounting for a total volume of 2.03$\,\m^3$. Based on discussions with the
two major suppliers, BTCP and SICCAS, and the actual prize
tag for the \INST{CMS}
calorimeter, a value of 4\,US\$/cm$^3$ will sum up to a total of 6.1\,M\euro. In
contrast to the typical offers of European and US companies, SICCAS has
indicated a significantly lower prize limit for BGO of 6\,US\$/$\cm^3$,
nevertheless increasing the total investment for crystals by 25\percent to
9.15\,M\euro.
There can be significant changes in both directions caused by the total
number of different shapes, the tolerances of dimensions and of surface
quality and acceptance limits of optical and scintillation properties.  

The development of appropriate photo sensors has concentrated on large
size APDs of 1$\,\cm^2$ active area. A first offer of the involved supplier
states 114\,\euro{} per sensor. Under the minimal assumption to achieve the
intended resolution with a single APD a total of 2.17\,M\euro{} has to be
considered and has to be doubled to 4.3\,M\euro, if two APDs have to be used. 
However, the solution with 2 APDs is by far more reliable and therefore preferable
taking into account the long envisaged lifetime and 
the long data taking periods of the experiment.

The scheme of the readout electronics, minimized with respect to size and
power consumption, can presently not be fixed. Uncertainties due to the
number of APDs per crystal, the deduction of energy and time information
and the practical limits on noise and dynamic range lead to a variation of
the costs per channel of almost 100\percent. A rough estimate for a single APD
per crystal amounts to 150\,\euro/crystal with a sum of 2.85\,M\euro{} as a lower limit to the total costs
including front-end electronics, ADC, signal transfer and bias voltage.
With 2 APDs on a crystal this may increase by a factor 1.4, leading to 210\,\euro/crystal.
Thus, the readout will contribute with a sum of 4\,M\euro{}.

In addition, a budget of 1\,M\euro{} should be added for development of prototype
detectors, mechanical components and electronics. \Reftbl{tab:main:cost} summarized the
estimated costs of the major components as discussed before.

%
\begin{table*}
\centering
\begin{tabular}{lrcr}
\hline\hline \\
\multicolumn{2}{l}{Component} & \multicolumn{2}{c}{Costs}\\
\multicolumn{2}{l}{} & Per piece & Total  [k\euro]\\
\hline
\multicolumn{2}{l}{Mechanical construction and cooling} & & 1\,000 \\
\multicolumn{4}{l}{19\,030 Scintillator crystals ($2.03\,\m^3$)} \\
& for PWO & 3\,\euro/$\cm^3$ & 6\,100 \\
& for BGO (opt) & 4.5\,\euro/$\cm^3$ & (9\,150) \\
\multicolumn{2}{l}{Photo sensor (2 APDs per crystal)} & 114\,\euro/APD & 4\,350 \\
\multicolumn{2}{l}{Readout electronics, cables, HV, ...} & 210\,\euro/crystal & 4\,000 \\
\multicolumn{2}{l}{Development and prototyping} &  & 700 \\
\hline
\multicolumn{2}{l}{Total} &  & 16\,150 \\
\hline\hline
\end{tabular}
\caption{Cost estimate for the target calorimeter.}
\label{tab:main:cost}
\end{table*}



==> exs/exs_req.tex <==
\section{Design Considerations}
\label{sec:exs:req}
Good recognition and reconstruction of multi-photon and lepton-pair channels
are of utmost importance for the success of the \Panda experiment. Low energy thresholds
and good energy and spatial resolution are important assets to achieve high yield and good background rejection.
Due to the high luminosity fast response and radition hardness are additional requirements which
have to be fulfilled. \Reftbl{tbl:req:summary} shows the detailled list of specifications for the EMC.
%
\begin{table*}[hbtp]
\begin{center}
\input{./req/req_table.tex}
\label{tbl:req:summary}
\end{center}
\end{table*}
%


==> panda_tdr_EMC_prod.tex <==
% FILE: panda_tpr_EMC_prod.tex
%
\cleardoublepage
\chapter{Production and Assembly}
\label{sec:prod}
%
% Text for this section
%
\input{./prod/planning}
%
% Bibliography for this chapter (remove %)
%
\newpage
\bibliographystyle{panda_tdr_lit}
\bibliography{./lit_emc}
%
% EOF: panda_tdr_EMC_prod.tex


==> prod/planning.tex <==
\section{Crystals}

\section{Avalanche Photodiodes}

\section{Vacuum Phototriodes}

\section{Electronics}
\label{sec:prod:elo} 

\section{Mechanics}

\section{Overall Timeline}
%
\Reffig{fig:prod:timeline} shows the overall timeline including the main tasks for the final design phase, the prototyping and production phase of the \TSEMC. The responsibilites for the various workpackages and tasks are listed in 
\Reftbl{tab:org:tasks} in \Refchap{sec:org} together with the institutions participating in executing the various tasks.

\begin{figure*}
\centering
\includegraphics[width=\dwidth]{./prod/emc_time}
\caption[Timeline for the EMC.]{Timeline for the EMC.}
\label{fig:prod:timeline}
\end{figure*}
%
%\clearpage
%
%
% EOF


==> req/requirements.tex <==
\section{Physics Objectives}
The envisaged physics program relies heavily on the capability to
measure photons with high energy, position and timing resolution over
a wide dynamic range starting at a few tens of MeV up to several GeV
energy. The reconstruction of the electromagnetic shower has to
deliver the energy as well as the point of impact of the photon with
high precision in a completely closed geometry. In particular the
identification of single photons as well as the coincident detection
of the decay photons from multi-meson exit channels relies on a high
and homogeneous efficiency. The invariant mass reconstruction requires
in addition the precise determination of the opening angle between the
decay photons, which can be achieved only by a highly granular
calorimeter. Choosing a compact scintillator material with a short
Moli\`ere radius, such as lead tungstate PbWO$_4$ or bismuth germanate
Bi$_4$Ge$_3$O$_{12}$, provides in addition a minimum occupancy of the
detector modules. This is true even in case of high charged and
neutral particle multiplicities considering heavy targets up to the
highest beam luminosities.

The expected high count rate, a geometrically compact design and
severe constraints on good energy and position resolution for the
detection of high energy photons require a homogeneous electromagnetic
calorimeter based on inorganic scintillator crystals. To minimize the
low energy threshold as well as the overall size, the calorimeter has
to be placed inside the coil of the superconducting solenoid. That
implies the readout of the scintillation light in a strong magnetic
field $<2\,\T$ and thus excludes the use of standard photomultiplier
tubes.
% which allow optimum
%light collection and maintain the fast response of a scintillator. 

Based on the physics objectives and the geometrical layout aiming for a
compact target spectrometer a fast scintillator material with short
radiation length and Moli\'ere radius becomes mandatory. 

The material of first choice is lead tungstate, PbWO$_4$ (PWO), a very
compact and radiation hard material. About ten years ago PWO has been
reinvented primarily for high energy applications and was chosen
consequently by the \INST{CMS} \cite{bib:emc:overview:ref1} and \INST{ALICE} \cite{bib:emc:overview:ref2}
collaborations at \INST{CERN}. The manufacturing process has been
optimized for large scale production. Timing on the level of $\approx
1\,\ns$ can be achieved using an appropriate readout with Avalanche Photo
Diodes (APDs). Due to expected annihilation rates of up to a few times
$10^7$/s, the possibility for fast timing matches well with the
requirement of a high count rate. Therefore, besides the
reconstruction of the electromagnetic shower it can deliver input for
fast trigger decisions, timing correlations between different detector
components and a very sensitive capability of background reduction.

Since the \Panda detector aims for the detection of photons well below
$20\,\mev$ energy, the present quality of the luminescence yield has
to be improved by at least a factor of five, which can partly be
achieved by operation at low temperatures $<-20\degrees$C. The
required improvement factor has been extrapolated from response
functions measured in the past for large size crystals of similar
dimensions but readout with photomultiplier tubes at temperatures only
slightly below room temperature \cite{bib:emc:overview:ref3}. It has been confirmed that,
even at medium energies, photon, electron, and hadron detection can be
achieved with good energy and excellent time resolution relying on
photomultiplier readout \cite{bib:emc:overview:ref4},\cite{bib:emc:overview:ref5}.  As a limiting factor, the
readout of the scintillation light via one or two large size APDs will
never cover the end face of the crystal completely. However, part of
the missing sensitivity due to the limited active area can be
compensated by the higher quantum efficiency of the sensor.

%Nevertheless, in spite of the significantly lower light yield ($\approx$
%10\percent of BGO) 

Bismuth germanate, Bi$_4$Ge$_3$O$_{12}$ (BGO), with a light yield larger
by a factor of $>\,$10, represents an alternative and backup
solution. The electromagnetic section of the former \INST{L3} detector at
\INST{CERN} used for the first time pure and doped crystals of $22\,X_0$
overall length \cite{bib:emc:overview:ref6} assembling a large fully closed calorimeter.
Nowadays BGO is primarily used for technical and medical applications,
since it delivers sufficient scintillation light even for low energy
radioactive sources. However, there are also disadvantages.
Timing and count-rate capabilities can never reach the level of PWO
due to its rise- and decay-times. These are longer at least by an order
of magnitude compared to PWO. It remains unclear if this has any implication 
on the operation in \Panda. It is one of the R\&D projects for BGO.
%  a significant amount of 
Moreover, R\&D will become necessary to verify homogeneity, radiation hardness and
the technology for mass production of large size crystals.
Also the question of a reliable supply remains open, as currently there
is only one supplier offering reasonable priced crystals.
%, if one has to consider BGO as an alternative.

Long term operation of the detector in an environment of a high integral
dose due to electromagnetic probes as well as charged and neutral hadrons
will have to cope with possible radiation damage of the scintillator
material and of the photo sensor, i.e.\ the APD. The present
considerations are guided by the large experience and technological
development within the CMS collaboration. However, in case of \Panda
significantly lower dose rates and integral doses can be expected in spite
of the much lower energy regime and interaction rates. A final estimate
based on realistic simulation can not be presented now.

\section{Geometrical Coverage and Dynamical Energy Range}
As outlined in the previous section the geometrical coverage of the
calorimeter section has to be as close as possible to $4\pi$.
This is to provide a significant efficiency for multi-photon exit channels
and a sufficient reduction of the background due to missing photons from
meson decays to make the identification of single photons possible.
The central area will be covered by the target
spectrometer consisting of a scintillator barrel closed by two annular
end caps. In backward direction an opening will be left for the
incoming beam. A larger window at forward angles will be covered by
the forward calorimeter located behind the dipole magnet (see \Refsec{sec:emc:forward}).

From the simulations of selected key reaction channels, which are
discussed in detail in \Refchap{sec:perf}, the acceptance range in
energy can be deduced. The upper limit of approximately $10\,\gev$
photon energy is set by the projectile energy range. The envisaged
lower limit of a few tens of $\mev$ has to be made reachable by the
detector quality. However, the final energy cut will depend on the
integral absorption of the material sandwich placed in front of the
calorimeter, caused by detector material, support structures and
additional layers for cooling and thermal shielding.

Details on the tolerable amount on dead material are not yet knwon and
will strongly depend on the final construction of all detector components.
Conversion directly in  front of the active calorimeter volume will have
the least impact.

\section{Energy, Position and Time Resolution}
The energy resolution of the electromagnetic calorimeter is determined
by the statistics of photo electrons collected in the photosensor and
the statistical fluctuations of the leakage or containment of the
electromagnetic shower within the detector. Therefore, the detector
material has to provide sufficient luminescence yield per
deposited energy unit. The containment of the shower energy has to be
guaranteed by sufficient depth, which ranges between 18 and 20 X$_0$
for the maximum energies, and a minimized dead space and material in
between adjacent elements. The individual crystal element has to allow
minimum energy thresholds in the order of 0.1-1\percent of the typical
photon energy.  Beside the contribution of statistics and electronics
noise to the overall resolution, given as 
\begin{equation}
\frac{\sigma_E}{E} = \frac{a}{\sqrt{E}}\oplus\frac{b}{E} \oplus c~~,
\end{equation}
the constant term $c$ reflects the accuracy of
inter-calibration but also time-instabilities and inhomogeneities. In
particular, the strong temperature dependence of the scintillation
process and the response of the APD photosensor cause a great
technological challenge.

The achievable energy resolution will depend on the size of the active
volume, which is composed of the direct or even next neighbours of the
directly hit calorimeter component. The acceptable cluster size will
depend on the multiplicity of reaction products and the occupancy of the
modules. However, the geometrical arrangement should foresee that the
electromagnetic probes are always impinging aligned to the crystal axis.
In addition, the experimental cluster size can be used to discriminate
electromagnetic showers and the narrow track of charged particles as long
as they do not initiate an electromagnetic shower.

The position resolution is primarily determined by the granularity and the
dimension of the crystal diameter with respect to the Moli\'ere radius R$_M$.
The proposed diameter close to R$_M$ will allow a position resolution better
than 10\percent of the crystal diameter, which will be $<2\,\mm$.

The compact design of the target calorimeter can not provide sufficient
resolution for particle/photon discrimination via time-of-flight. However,
the envisaged and in case of PWO achievable time resolution of $\approx 1\,\ns$ for
relevant photon energies can have significant advantages, which have not
been considered in the basic Monte Carlo simulations. Presently operating
calorimeters such as the \INST{Crystal Barrel} composed of CsI(Tl) \cite{bib:emc:overview:ref7} and
the NaI(Tl) \INST{Crystal Ball} \cite{bib:emc:overview:ref8} rely heavily on fast triggering
additional detector components due to their slow read-out and slow
scintillation response. Besides a fast trigger input, the reachable time
resolution provides strong selectivity to correlate additional detectors
or reduce background. The consequences on the read-out circuits have not
been investigated yet.


\section{Count-Rate and Occupancy Limits}

The count-rate limit is primarily determined by the luminescence
properties of the chosen scintillator. In that respect PbWO$_4$ represents
the optimum material due to its extremely short decay kinetics, which is
dominated by the prominent component of $\tau = 6.5\,\ns$ (97\percent). Even an operation
foreseen at lower temperatures will guarantee the complete light
collection within a gate width of $< 100\,\ns$. Therefore, even an event rate
of 10$^7$ annihilations per second will not lead to pile-up effects in the
scintillator. The read-out via APDs or vacuum triodes, both in combination
with charge sensitive preamplifiers and subsequent shaping, might reduce
the count rate capabilities. A sufficiently long shaping time might become
necessary to optimize the signal-to-noise ratio in particular for low
energy signals. Experimental results are presently not yet available.

The foreseen segmentation of the target calorimeter in elements with a
diameter comparable to the Moli\'ere radius will not impose a limit on the
acceptable occupancy for antiproton induced reactions on hydrogen or
helium. The expected values for heavy targets have to be still simulated.

\section{Radiation Hardness}
\label{sec:req:rad}

The long year development for the electromagnetic calorimeter ECAL of \INST{CMS}
provides detailed experimental data for the radiation hardness with
respect to high radiation dose rates as well as a high integral dose
extrapolated for a typical 10 year operation. A rough estimate based on
the expected luminosity of the \INST{HESR} delivers a significantly lower
radiation yield, but detailed calculations are not net present due to the
large complexity and several unknown facts.

The investigation of the sensitivity of PbWO$_4$ to the damage due to
electromagnetic and hadronic probes shows, that the degradation is
primarily caused by a reduction of the optical transmission of the crystal
due to color center formation. No permanent damage due to structure
defects have been identified. The moderate recovery time leads to a
saturation of the transmission loss to a level of typically 95 to 97\percent for
the radiation dose of \INST{LHC} operation. Since the \INST{HESR} luminosity is lower by
orders of magnitude, only a long term deterioration of the crystal
performance has to be taken into account, which can be monitored during
off-line data analysis. \INST{CMS} studies of the radiation damage due to
neutrons or protons have shown very contrary results, probably due to
crystal samples of not identical quality. Performed first irradiation
measurements impinging with 90$\,\mev$ protons, see \Refsec{sec:scint:pwo:rad} for
details, confirm sufficient radiation hardness.

The development of radiation hard APDs has been a major task for \INST{CMS},
which has been successfully performed in case of small size APDs of
($5\times 5$)$\,\mm^2$ active area. In particular the manufacturing process of the surface
structures was essential to stabilize the functionality. Based on that
experience further R\&D are necessary to establish similar quality for
large size sensors, which are mandatory for \Panda. The tuning process for
\INST{CMS} requires a pre-irradiation of the sensors to sort out weak components
and to guarantee the long term operation.  As a negative consequence, a
significant increase of the dark current has to be accepted, which might
cause limitations for the measurement of photons in the MeV range due to a
large noise level. The expected significantly lower dose rates for \Panda
will hopefully make such treatments obsolete. Nevertheless, detailed
studies of the damage due to highly ionizing low energy protons, generated
for example via (n,p)-reactions in the crystal, have to be performed and
have been started already (see \Refsec{sec:photo:APD}). Additional complication
might arise when operation at lower temperature might block or delay
annealing processes in the silicon.



==> scint/scint_alt.tex <==
The concept of \Panda places the target calorimeter inside the
superconducting coil of the solenoid. Therefore, the basic requirement of any appropriate scintillator material
has to be its compactness to minimize the radial thickness of the calorimeter
barrel \cite{bib:emc:scint:alt16,bib:emc:scint:alt17}. Presently and even in the near future, there are no materials besides PWO available,
which are developed for mass production of large and extremely homogeneous crystals.

\begin{table*}
\begin{center}
\begin{tabular}{lcccc}
\hline\hline
\multicolumn{2}{c}{Parameter} & CeF$_3$ & LSO/LYSO:Ce & BGO \\
\hline
$\rho$           & g/cm$^{3}$             & 6.16 & 7.40 & 7.13 \\
$X_0$            & $\cm$                  & 1.77 & 1.14 & 1.12 \\
$R_M$            & $\cm$                  & 2.6  & 2.3  & 2.3  \\
$\tau$$_{decay}$  & $\ns$                  & 30   & 40   & 300  \\
$\lambda$$_{max}$ & $\nm$                  & 330  & 420  & 480  \\
$n$              &                        & 1.63 & 1.82 & 2.15 \\
relative LY & \percent($LY$ NaI)          & 10   & 75   & 9    \\
hygroscopic      &                        & no   & no   &  no  \\
dLY/dT       &  \percent/$\degC$    & 0.1  & -0.3 &  -1.6 \\
\hline\hline
\end{tabular}
\caption[Properties of CeF$_{3}$, LSO/LYSO:Ce and BGO]{Relevant properties of CeF$_{3}$, LSO/LYSO:Ce and BGO.}
\label{tab:scint:alt:prop}
\end{center}
\end{table*}

Of the materials listed above Bismuth Germanate (Bi$_4$Ge$_3$O$_{12}$, BGO) is a well known scintillator
material since many decades~\cite{bib:emc:alt1}. It has been applied in several experiments, like \INST{L3} at \INST{CERN} or \INST{GRAAL}at Grenoble, providing well performing electromagnetic calorimeters ~\cite{bib:emc:alt2,bib:emc:alt3,bib:emc:alt4}. However, presently it is only used in large quantities but small samples for medical applications such as Positron-Electron-Tomography (PET) scanners ~\cite{bib:emc:alt5}.

The properties of BGO, listed in \Reftbl{tab:scint:alt:prop}, allow for the design of a very compact calorimeter. The
light yield is about a factor of 2 higher than cooled PWO crystals. The emission wavelength is well suited for an efficient readout with photo or avalanche diodes. However, the moderate decay time imposes a strong limitation on the necessary high rate capability for the envisaged interaction rate of 10$^{7}$/s of \Panda. In addition, it excludes in general any option for the generation of a fast timing information on the level of $\leq$1--2ns or even below for higher energies.

Concerning the radiation hardness, which has not been a major issue for the former applications, controversial results are reported in the literature. Some authors report recovery times in the order of days or online recovery by exposure
to intense light from fluorescent lamps at short wavelengths \cite{bib:emc:alt6,bib:emc:alt7,bib:emc:alt8,bib:emc:alt9}. Since most of these studies are rather old, an update with new studies using full size scintillation crystals produced recently would become necessary.

CeF$_{3}$ has been invented already in 1989 by D. F. Anderson \cite{bib:emc:scint:alt10} and
identified as a fast scintillator with maximum emission wavelength between
310 and 340nm. The luminescence process is dominated by radiative transitions of Ce$^{3+}$ ions, which explains the fast decay time of $\sim$30na and the insensitivity to temperature changes. The luminescence yield is
comparable or even higher than the fast component of BaF$_{2}$, corresponding to approximately 10\percent of  NaI(Tl) as a reference. Since the crystal matrix is extremely radiation hard, it was considered for the \INST{CMS} calorimeter
during a long period of R$\&$D, supported by the short radiation length and Moli\'ere radius, respectively. However, homogeneous crystal samples beyond 10X$_{0}$ length, grown by the Bridgeman method, have never been produced with
adequate quality.

Detailed studies of the response function \cite{bib:emc:scint:alt11} to low energy protons and high energy photons have documented excellent time and energy resolutions, which are limited only in case of the reconstruction of the
electromagnetic shower energy by the inhomogeneity of the available crystals. The way to improvement is by optimization of the manufacturing process.

However, the implementation of CeF$_{3}$ has not been considered. It would on one hand double the radial thickness of the calorimeter shell. On the other hand, the effective light yield would be degraded due to the mismatch of the emission wavelength in the near UV with the optimum quantum efficiency of APDs.

In the last decade cerium doped silicate based heavy crystal scintillators have been developed for medical applications, which require high light output for low energy $\gamma$-ray detection and high density to allow for small crystal units. Mass production of small crystals of Gd$_{2}$SiO$_{5}$ (GSO), Lu$_{2}$SiO$_{5}$ (LSO) and Lu$_{2(1-X)}$Y$_{2X}$SiO$_{5}$ (LYSO) has been established in the meantime. Because of the high stopping power and fast and bright luminescence, the latter material has also attracted interest in calorimetry. However, the need for large homogeneous samples and the
presently high costs, partly justified by the high melting point, are retarding the R$\&$D.

LYSO, which has almost identical physical and scintillation properties as LSO and shows identical emission, excitation and optical transmittance spectra, has been recently produced in samples up to 20cm length \cite{bib:emc:scint:alt12,bib:emc:scint:alt13,bib:emc:scint:alt14,bib:emc:scint:alt15}. The light output is about 4 times of BGO but with a decay time shorter by one order of magnitude, determined by the Ce-activation. Detailed studies even within the PANDA-collaboration have been performed and response functions have been obtained even for high-energy photons up to 500MeV \cite{bib:emc:scint:alt14}. Aiming for applications for the next generation of homogeneous calorimeters, detailed studies of full size crystals with respect to homogeneity, scintillation processes and radiation hardness are part of a research program promoted by a group at Caltech \cite{bib:emc:scint:alt15}.




==> sim/simulationsWithHitRates.tex <==

The simulation studies described in the following are focused on the expected performance of 
the planned EMC with respect to the energy and spatial resolution of reconstructed photons, to
the capability of an electron hadron separation, and also to the feasibility of the planned 
physics program of \Panda. A couple of benchmark studies based on accurate simulations will be 
presented, where the necessity of the planned EMC will be highlighted. Due to the
fact that most of the physics channels have very low cross sections \-- typically 
between pb and nb \-- , a background
rejection power up to $10^9$ has to be achieved. This requires an electromagnetic 
calorimeter which allows an accurate photon reconstruction within the energy 
rage between 10$\,\mev$ and 15$\,\gev$, and an effective and an almost clean electron hadron 
separation. 
  
       
\section{Offline Software}
The offline software has been devised for detailed design studies of the \Panda detector
and for the preparation of the \Panda Physics Book, which will be 
published by September 2008. It follows an object oriented approach, and most of the code
is written in C++. Several proofed software tools and packages from other 
HEP experiments have been adapted to the \Panda needs and are in use. The software contains
\begin{itemize}
\item event generators with proper decay models for all particles and resonances involved in 
the individual physics channels as well as in the relevant background channels,
\item particle tracking through the complete \Panda detector by using the GEANT4 transport
code \cite{bib:sim:Allison, bib:sim:Agostinelli},
\item a digitization which models the signals and the signal processing in the 
front-end-electronics of the individual detectors,
\item the reconstruction of charged and neutral particles, comprising a particle identification
that provides lists of particle candidates for the final physics analysis, and
\item user friendly high level analysis tools with the purpose to make use of vertex
and kinematical fits and to reconstruct even complicate decay trees in an easy way.
\end{itemize}  

\subsection{Photon Reconstruction}
\subsubsection{Reconstruction Algorithm} \label{sec:sim:recoalgo}
A photon hitting the EMC produces an electromagnetic shower which, in general, extends
over several crystals. A contiguous area of such crystals is called a cluster.

The energy deposits and the positions of all hit  crystals allow a 
determination of the four vector of the initial photon. Most of the EMC reconstruction
code used in the offline software is based on the cluster finding and bump splitting 
algorithms which were developed and successfully applied by the BaBar experiment 
\cite{bib:sim:BaBarDetector, bib:sim:Strother}.

The first step of the cluster reconstruction is the finding of a contiguous area of
crystals with energy deposit. The algorithm starts with the highest energy crystal.
Its neighbors are then added to a list of potential inclusion of a cluster if the
energy deposit is above a certain threshold $\extl$. The same procedure follows
with the neighbors of the new crystals and continues until no more of the neighboring
crystals are above the required energy threshold. Finally a cluster is accepted if
the total energy deposit in the contiguous area is above $\ecl$.

A cluster can be formed by more than one particle if the angular 
distances of the particles are small. In this case the cluster has to be subdivided
into regions which can be associated with the individual particles. This procedure 
is called the bump splitting. A bump is defined by a local maximum inside the cluster:  
The energy deposit of one crystal ($E_{LocalMax}$) must be above $\emax$, while all neighbor
crystals have smaller energies. In addition the highest energy $E_{NMax}$ of any of the 
$N$ neighboring crystals must fulfill the following requirement:
\begin{eqnarray}
 0.5\,(N-2.5) \, > \, E_{NMax} \, / \,  E_{LocalMax}
\end{eqnarray} 
The total cluster energy is then shared between the bumps which takes the shower shape of the 
cluster into account. For this step an iterative algorithm is used, where each crystal
becomes a weight, $w_i$, so that the bump energy is defined as 
$E_{bump}= \sum_{i} \, w_i \, E_i$. $E_i$ represents the energy deposit in the ith crystal 
and the sum runs over all crystals within the cluster. 
The crystal weight for each bump is calculated by  
\begin{eqnarray} 
w_i = \frac{E_i \, exp(-2.5 \, r_i\, / \,r_m)}
            {\sum_{j} E_j \, exp(-2.5 \, r_j\, / \,r_m)}
\end{eqnarray}
, with
\begin{itemize}
\item $r_m$ = Moli\`ere radius of the crystal material,
\item  $r_i$,$r_j$ = distance of the ith and jth crystal to the centroid of the bump and
\item  index $j$ runs over all crystals. 
\end{itemize} 
The procedure is then iterated, whereby the centroid position is determined with the weights
of the previous iteration until the bump centroid is stable within a tolerance of 1$\,\mm$.
       
The spatial position of a bump is calculated via a center-of-gravity method. Due to the fact 
that the radial energy distribution originating from a photon decreases mainly exponentially, 
a logarithmic weighting with
\begin{eqnarray}
  W_i \, = \, max(0, A(E_{bump}) \, + \, ln\,(E_i / E_{bump}))
\end{eqnarray}
 was chosen, where only crystals with positive weights are used. The energy dependent factor 
$A(E_{bump})$ varies between 2.1 for the lowest possible and 3.6 for the highest possible 
photon energies.           
   
\subsubsection{Digitization of the crystal readout} 
\label{sec:sim:digi}
A detailed simulation of the EMC digitization has to take into account the signal waveforms
and the digitization process. For performance reasons a more 
simplified method has been applied in the simulation studies, which is based on an effective 
smearing of the extracted Monte Carlo energy deposits. 
Reasonable properties of $PbWO_4$ at the operational temperature of -25$^0$C have been considered. 
A Gaussian distribution of $\sigma$ = 1$\,\mev$ has been used for the constant electronics noise. 
The statistical fluctuations were estimated by 80 phe/\mev produced in the LAAPD. Based on this
estimate an excess noise factor of 1.38 has been used which corresponds to the measurements with 
the first LAAPD 'normal C' prototype at an internal gain of $M=50$ (see 
\Refsec{sec:photo:APD:Char:ENF}). This results in a photo statistic noise term 
of 0.41\% /$\sqrt{E}$.  

\paragraph{Comparison with 3x3 crystal array measurements}

In order to demonstrate that the digitization is described sufficiently with this simplified
method, a comparison with the 3x3 crystal array measurements (see \Refsec{subchap:perform:energy-apd})
has been done. The obtained line shapes (\Reffig{fig:perf:perf16} and \Reffig{fig:perf:perf17}) 
and energy resolution as a function of incident photon energy (\Reffig{fig:perf:perf19}) are based
on  measurements at the operational temperature of 0$^0$C.

The simulations have been realized with an 3x3 array and crystal dimensions of 2x2x20$\,$cm$^3$. Photons 
with discrete energies between 40.9$\,\mev$ and 1$\,\gev$ were shot in the center of the innermost 
crystal. To consider the crystal temperature of 0$^0$C the digitization has been done with only 
40 phe/\mev instead of 80 phe/\mev produced in the LAAPD. The resulting line shape at the photon 
energy of 674.5$\,\mev$ is illustrated in \Reffig{fig:sim:reso3x3_674}. The fit with the Novosibirsk 
function defined by
\begin{eqnarray}
f(E) = A_S \exp ( -0.5 { \ln^2 [1 + \Lambda \tau \cdot (E - E_0) ] / \tau^2 + \tau^2 } ) \nonumber
\end{eqnarray}
,with
\begin{itemize}
\item $\Lambda = \, \sinh ( \, \tau \, \sqrt{\, \ln 4} ) / ( \, \sigma \, \tau \, \sqrt{\ln 4} )$,
\item $E_0\,$= peak position,
\item $\sigma\,$= width, and
\item $\tau\,$= tail parameter
\end{itemize}
yields to a resoultion of $\sigma/E\;=\;2.63\,$\% which is in good agreement
with the measurements (see \Reffig{fig:perf:perf17}). Moreover the energy resolution as a function of
the incident photon energy can be reproduced very well. \Reffig{fig:sim:reso3x3_all} shows the results 
obtained with the simulations and \Reffig{fig:perf:perf19} is the corresponding histogram of the measurements.  
       

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/reso3x3_674}
\caption[Simulated line shape of the 3x3 crystal matrix at the photon energy of 674.5$\,\mev$.]
{Simulated line shape of the 3x3 crystal matrix at the photon energy of 674.5$\,\mev$. The fit with
the Novosibirsk function results in an energy resolution of $\sigma/E\,=\,2.63\,$\% }
\label{fig:sim:reso3x3_674}
\end{center}
\end{figure}    

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/reso3x3_all}
\caption[Simulated energy resolution as a function of incident photon energy between 40.9$\,\mev$
and 674.5$\,\mev$ for a 3x3 crystal array.]
{Simulated energy resolution as a function of incident photon energy between 40.9$\,\mev$
and 1$\,\gev$ for a 3x3 crystal array.}
\label{fig:sim:reso3x3_all}
\end{center}
\end{figure} 

\subsubsection{Reconstruction Thresholds}\label{sec:sim:recothresh}
In order to detect low energetic photons and to 
achieve a good energy resolution, the three photon reconstruction thresholds should be set as 
low as possible. On the other hand the thresholds must be sufficiently high to suppress the 
misleading
reconstruction of photons from the noise of the crystal readout and from statistical fluctuations 
of the 
electromagnetic showers. Based on the properties of the \Panda EMC
(see \Refsec{sec:sim:digi}) the following thresholds were chosen:

\begin{itemize}
\item $\extl\,=\,3\,\mev$
\item $\ecl\,=\,10\,\mev$
\item $\emax\,=\,20\,\mev$  .
\end{itemize}

As already discussed in \Refsec{sec:ethres} the ability to identify photons down to 
approximately $10\,\mev$ plays an essential role for 
\Panda. A lot of channels \--- especially in the charmonium sector like 
$\bar{p} p \rightarrow \eta_c \rightarrow \gamma \gamma$,
$\bar{p} p \rightarrow h_c  \rightarrow \eta_c \gamma$ or  $\bar{p} p \rightarrow J\psi \gamma$ 
\--- require an accurate and clean reconstruction of isolated photons. The main background channels 
here have the same final states with just the isolated photon being replaced by a $\pi^0$. 
If one low energetic photon from a $\pi^0$ decay gets lost, the background event will
be misidentified. The cross sections for the 
background channels usually are a few orders of magnitudes higher than for the channels of interest.
Therefore an efficient identification of $\pi^0$'s is mandatory for this important part of the 
physics program of \Panda. \Reffig{fig:pizloss} in \Refsec{sec:ethres} shows the upper limit for 
the 
identification of $\pi^0$'s with respect to different photon thresholds.
While roughly 1\% of the $\pi^0$'s get lost with for a threshold of 10$\,\mev$, the 
misidentification increases by one order of magnitude for the scenario where photons below 
30$\,\mev$ can not be detected.          
    
%\begin{figure}[htb]
%\begin{center}
%\includegraphics[width=1.15\swidth]{./sim/pi0Efficiency}
%\caption[$\pi^0$ reconstruction efficiencies for different photon thresholds.]
%{$\pi^0$ reconstruction efficiencies for different photon thresholds.}
%\label{fig:sim:pieff}
%\end{center}
%\end{figure} 
 


\subsubsection{Leakage Corrections}
Because of shower leakages particularly in the crystal gaps, the sum of the 
energy deposited in the crystals in general is a few percent less than the energy of the
incident photon. The reconstructed energy of the photon is expressed as a product
of the total measured energy deposit and a correction function which depends 
logarithmically on the energy and \--- due to the layout of the \Panda EMC \--- also on 
the polar angle. Single photon Monte Carlo simulations have been carried out to determine the
parameters of the correction function $E_{\gamma,cor} = E * f(ln E,\Theta)$ with

\begin{eqnarray}
f(ln E,\Theta) = exp( a_0 + a_1\,ln E + a_2 \,ln^2 E + a_3 \,ln^3 E \nonumber\\
                   + a_4 \, cos(\Theta)+ a_5 \, cos^2(\Theta) + a_6 \, cos^3(\Theta) \nonumber\\
                  + a_7 \,cos^4(\Theta) + a_8 \, cos^5(\Theta) \nonumber\\
                  + a_9 \, ln E \, cos(\Theta) ) \nonumber 
\end{eqnarray} 

\Reffig{fig:sim:leakCorr} shows the result for the barrel part in the $\Theta$ range 
between 22 and 90 $deg$.  

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/corBarrel}
\caption[Leakage correction function for the barrel EMC in the $\Theta$ range 
between 22 and 90 $deg$ ]
{Leakage correction function for the barrel EMC in the $\Theta$ range 
between 22 and 90 $deg$.}
\label{fig:sim:leakCorr}
\end{center}
\end{figure} 


\subsubsection{Energy and Spatial Resolution}

The energy resolution of the EMC strongly depends on the length of the crystals. 
A sufficient containment of the electromagnetic shower within the detector and
marginal fluctuations of the shower leakages must be guaranteed for the detection 
of photons with energies up to 15$\,\gev$. \Reffig{fig:sim:eResol} compares the simulation
results for the foreseen \Panda EMC equipped with crystals of 15 cm, 17 cm and
20 cm length. While the resolution for low energetic photons \--- below 300$\,\mev$ \--- is 
nearly 
the same for all three scenarios, the performance becomes significantly better for higher 
energetic photons with an increasing crystal length. The 20 cm setup yields in an energy 
resolution of 1.5\% for 1$\,\gev$ photons, and of even below 1\% for 
photons above 3$\,\gev$.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/Ereso}
\caption[Energy resolution for three different crystal length scenarios. ]
{Comparison of the photon energy resolution for three different crystal
lengths. The resolution for 15 cm crystals is illustrated by circles, for 17 cm 
by rectangles, and the 20 cm scenario is shown with triangles.}
\label{fig:sim:eResol}
\end{center}
\end{figure}

As already described in \ref{sec:sim:digi} and \ref{sec:sim:recothresh} the choice of the
single crystal threshold $\extl$, which is driven by the electronics noise term, strongly effects
the resolution. Three different scenarios have been investigated: \Reffig{fig:sim:eResolThreshold}
compares the achievable resolution for the most realistic scenario with a noise term of $\sigma$ = 1$\,\mev$
and a single crystal reconstruction threshold of $\extl=3\,\mev$ with a worse case 
($\sigma$ = 3 $\mev$, $\extl=9$ $\mev$) and a better case ($\sigma\,= \,0.5 \,\mev$, $\extl=1.5\,\mev$). 
While the maximal 
improvement for the better case is just 20\% for the lowest photon energies, the degradation
in the worse case increases by more than a factor of 2. This result demonstrates clearly
that the single crystal threshold has a strong influence on the energy resolution.


\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/Ereso_threshold}
\caption[Comparison of the energy resolutions for three different single crystal reconstruction 
thresholds. ]
{Comparison of the energy resolutions for three different single crystal reconstruction thresholds. 
The most realistic scenario with a noise term of $\sigma \, = \,1 \, \mev$
and a single crystal threshold of $\extl=3\,\mev$ is illustrated by triangles, a worse case
($\sigma \, = \, 3 \mev$, $\extl \, = \, 9 \, \mev$) by circles and the better case ($\sigma \, = \, 0.5 \, \mev$, 
$\extl \,= \, 1.5 \, \mev$) by rectangles.}
\label{fig:sim:eResolThreshold}
\end{center}
\end{figure}


The high granularity of the planned EMC provides an excellent position reconstruction 
of the detected photons. The accuracy of the spatial coordinates is
preliminary determined by the dimension of the crystal size with respect 
to the Moli\`ere radius. \Reffig{fig:sim:posResol} shows the resolution in x direction 
for photons up to 3$\,\gev$. A $\sigma_x$-resolution of less than 0.3 cm can be obtained 
for energies above 1$\,\gev$. This corresponds to roughly 10\% of the crystal size.
For lower energies the position becomes worse due to the fact that
the electromagnetic shower is contained in only few crystals. In the worst case
of only one contributed crystal the x-position can be reconstructed within an 
imprecision of 0.5-0.6 cm.

   

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/PosReso}
\caption[Position resolution in x-direction for photons below 3$\,\gev$. ]
{Position resolution in x-direction for photons below 3$\,\gev$.}
\label{fig:sim:posResol}
\end{center}
\end{figure}


\subsection{Electron Identification}
Electron identification will play an essential role for most of the physics program of 
\Panda. An 
accurate and clean measurement of the $J/\Psi$ decay in $e^+ \, e^-$ is needed for many  
channels in the charmonium sector as well as for the study of the 
$\bar{p}$ annihilation in nuclear matter like the reaction $\pbarp \, \to \, J/\Psi X$.
In addition the determination of electromagnetic form factors of the proton via 
$\pbarp \, \to \,e^+ \,e^- $ requires a suppression of the main background channel
$\pbarp \, \to \, \pi^+ \, \pi^-$ in the order of $10^8$.

The EMC is designed for the detection of photons, is also the most powerful
detector for an efficient and clean identification of electrons. 
The character of an
electromagnetic shower is distinctive for electrons, muons and hadrons. The most suitable
property is the deposited energy in the calorimeter. While muons and hadrons in 
general loose only
a certain fraction of their kinetic energy by ionization processes, electrons deposit
their complete energy in an electromagnetic shower. The 
ratio of the measured energy deposit in the calorimeter to the reconstructed track momentum 
($E/p$) will be approximately unity. Due to the fact that hadronic 
interactions within the crystals 
can take place, hadrons can also have a higher $E/p$ ratio than expected from ionization.
Figure \Reffig{fig:sim:eOpElectronsPions} shows the reconstructed $E/p$ fraction for electrons and pions
as a function of momentum.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/EOverP_el_pi_v1}
\caption[E/p versus track momentum for electrons and pions]
{E/p versus track momentum for electrons (green) and pions (black) in the momentum 
range between 0.3$\,\gevc$ and 5$\,\gevc$.}
\label{fig:sim:eOpElectronsPions}
\end{center}
\end{figure}      

Furthermore the shower shape of a cluster is helpful to 
distinguish between electrons, muons and hadrons. Since the chosen size of the crystals 
corresponds to the Moli\`ere radius of lead tungstate, the largest fraction of
an electromagnetic shower originating from an electron is contained in just a few 
crystals. Instead, an hadronic shower with a similar energy deposit is less concentrated.
These differences are reflected in the shower shape of the cluster, which can be 
characterized by the following properties:
\begin{itemize}
\item $E_1/E_9$ which is the ratio of the energy deposited in the central crystal and in 
the 3$\times$3 crystal array containing the central crystal and the first innermost ring.
Also the ratio between $E_9$ and the energy deposit in the 
5$\times$5 crystal array  $E_{25}$ is useful for electron identification.    
 \item The lateral moment of the cluster defined by
      $mom_{LAT} = \frac{\sum_{i=3}^n E_i r_i^2}{\sum_{i=3}^n E_i r_i^2 + E_1 r_0^2 +  E_2 r_0^2}$ with
\begin{itemize}
\item n: number of crystals associated to the shower.
\item $E_i$: deposited energy in the i-th crystal with $E_1 \geq E_2 \geq ... \geq E_n$.
\item $r_i$: lateral distance between the central and the i-th crystal.
\item $r_0$: approximately the average distance between two crystals. 
\end{itemize}
\item A set of zernike moments \cite{bib:sim:zernike} which describe the energy distribution within a 
cluster by
radial and angular dependent polynomials. An example is given in \Reffig{fig:sim:zernike31} 
where the zernike moment 31 is illustrated for each particle type.  
\end{itemize}


\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/zernike31}
\caption[Zernike moment 31 for electrons, muons and hadrons.]
{Zernike 31 moment for electrons, muons and hadrons.}
\label{fig:sim:zernike31}
\end{center}
\end{figure}

Due to the fact that a lot of partially correlated EMC properties are suitable for electron 
identification, a Multilayer 
Perceptron (MLP) has been applied. The advantage of a neural network is that it can 
provide a correlation between a set of input variables and one or several output 
variables without any knowledge of how the output formally depends on the input. Such
techniques are also successfully used by other HEP experiments \cite{bib:sim:Abramowicz, bib:sim:Breton:1995rg}. 

The
training of the MLP has been done with a data set of 850.000 single tracks for each 
particle species (e, $\mu$, $\pi$, K and p) in the momentum range between 200$\,mevc$ 
and 10$\,\gevc$ in such a way  that the output values are constrained to be 1 for 
electrons and -1 for all other particle types. 10 input variables in total have been
used, namely $E/p$, $p$, the polar angle $\Theta$ of the cluster, and 7 shower 
shape parameters
($E_1/E_9$, $E_9/E_{25}$, the lateral moment of the shower and 4 zernike moments). The
response of the trained network to a test data set of single particles in the 
momentum rage between 300$\,mevc$ and 5$\,\gevc$ is illustrated in \Reffig{fig:sim:nno}. 
The logarithmically scaled histogram shows that an almost clean electron recognition with a
quite small contamination of muons and hadrons can be obtained by applying a cut on the network output. 

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/nno}
\caption[MLP output for electrons and the other particle species 
in the momentum range between 300$\,mevc$ and 5$\,\gevc$.]
{MLP output for electrons and the other particle species 
in the momentum range between 300$\,mevc$ and 5$\,\gevc$.}
\label{fig:sim:nno}
\end{center}
\end{figure}

The global PID, which combines the PID informations of the individual sub-detectors, has
been realized with the standard likelihood method. Each sub-detector provides probabilities
for the different particle species, and thus a correlation between the network output and the PID 
likelihood of the EMC has been calculated. \Reffig{fig:sim:lhEMC} shows the electron efficiency 
and contamination rate as a function of momentum achieved  by requiring an 
electron likelihood fraction of the EMC of more than 95\%.
For momenta above 1$\,\gevc$ one can see that the electron efficiency is greater than 98\%
while the contamination by other particles is substantially less than 1\%. 
For momenta below 1$\,\gevc$ instead the electron identification obtained with just the EMC 
is quite bad and not sufficient.
 
\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/efficiency_lhEmc095}
\caption[Electron efficiency and contamination rate for muons, pions,
 kaons and protons in different momentum ranges by using the EMC informations.]
{Electron efficiency and contamination rate for muons, pions,
 kaons and protons in different momentum ranges by using the EMC informations.}
\label{fig:sim:lhEMC}
\end{center}
\end{figure}

A good electron-Id efficiency and small contamination rates can be achieved by taking
into consideration additional sub-detectors (MVD, Cerenkov detectors and muon counters) 
(\Reffig{fig:sim:lhAll}). By applying a 99.5\% cut
on the combined likelihood fraction, the electron efficiency 
becomes better than 98\% while the pion misidentification is just on the $10^{-3}$ level over 
the whole momentum range. The contamination rates for muons, kaons and protons are 
negligible.
     
\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/efficiency_lhAll_0995}
\caption[Electron efficiency and contamination rate for muons, pions,
 kaons and protons in different momentum ranges by using the combined PID informations.]
{Electron efficiency and contamination rate for muons, pions,
 kaons and protons in different momentum ranges by using the combined PID informations.}
\label{fig:sim:lhAll}
\end{center}
\end{figure}
 

\section{Material budget in front of the EMC}
The reconstruction efficiency as well as the energy and spatial resolution of the EMC  
are affected by the interaction of particles with material in front of the calorimeter.
While the dominant interaction process for photons in the energy range of interest
is $e^+\,e^-$ pair production, electrons lose energy mainly via 
Bremsstrahlung ($e \, \to \, e \, \gamma$). \Reffig{fig:sim:x0} illustrates the 
material budget in front of the individual sub-detectors in units of radiation lengths
as a function of $\Theta$.
The largest contribution to the material budget in front of the EMC comes from the
Cerenkov detectors, which consist of quartz radiators of 1-2 $cm$ thickness. 
This corresponds to 17\% to 50\% of a radiation length, depending on the polar angle.
     
\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/X0}
\caption[Amount of material in front of the EMC.]
{Material in front of the EMC in units of a radiation length $X_0$ as a function of the 
polar angle $\Theta$.}
\label{fig:sim:x0}
\end{center}
\end{figure}

\subsection{DIRC preshower}
As \Reffig{fig:sim:x0} shows, the DIRC detector contributes most to the material budget
in front of the EMC. Therefore detailed Monte Carlo studies have been done
to investigate the impact of this device on the $\gamma$ reconstruction 
efficiency and energy resolution. \Reffig{fig:sim:gammaConfDIRC} represents the 
$\gamma$ conversion probability in the DIRC for
1$\,\gev$ photons generated homogeneously in the $\Theta$ range 
between 22 deg and 145 deg. While 15\% of the photons convert at the polar angle of 90 deg,
the DIRC preshower probability increases up to 27\% at 22 deg. 
        
\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/gammaConversionDIRC}
\caption[$\gamma$ conversion probability in the DIRC as a function of $\Theta$]
{$\gamma$ conversion probability in the DIRC as a function of $\Theta$}
\label{fig:sim:gammaConfDIRC}
\end{center}
\end{figure}   

DIRC preshowers mainly lead to a degradation of the energy 
resolution. A comparison of the reconstructed energies for 1$\,\gev$ photons 
with and without DIRC preshowers is shown in \Reffig{fig:sim:resPreshower}. While
the energy distribution for non preshower photons can be well described by a 
Gaussian function with $\sigma(\Delta E/E)$ \, = \, 2\%, 
the distribution for DIRC preshower clusters becomes significantly worse. Due to the fact 
that a fraction of the photon 
energy is deposited in the quartz bars, a broad and asymmetric distribution with a huge
low energy tail shows up.
      
\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/gammaResPreshower}
\caption[Reconstructed energy of 1$\,\gev$ photons with and without DIRC preshowers.]
{Reconstructed energy of 1$\,\gev$ photons without (black circles) and with (red triangles)
 DIRC preshowers. For a better comparison the plot with DIRC preshowers are scaled by a factor of 4.87.}
\label{fig:sim:resPreshower}
\end{center}
\end{figure} 


\subsubsection{Outlook: Preshower recognition and energy correction.}
If the Cerenkov light originating from the produced $e^+$ $e^-$ pairs get measured, 
the number of detected 
Cerenkov photons provides a measure for the energy loss, and thus an energy correction 
of such clusters could be feasible. A DIRC preshower recognition with an additional 
energy correction would yield in a better performance of the photon reconstruction.

Based upon recent investigations for the BaBar experiment, it is expected to achieve
a DIRC preshower detection efficiency of better than 50\% and an improvement for the photon
energy resolution of more than 1\% \cite{bib:sim:Adametz}.
      

\section{Crystal Hit Rates and absorbed Energy Dose}
The single crystal rates for the proposed running conditions had been
simulated using the Dual Parton Model (DPM) as generator for primary events.
The beam momentum of 15~GeV/c was used to evaluate the highest load for
$\pbarp \, \to \, X$ interactions.
A full tracking of the primary generated events through the whole
\Panda detector was simulated using GEANT3/4 .
The results are scaled
to the canonical interaction rate of 10$^7$ primary
events/s corresponding to an average luminosity of $2\times 10^{32}$ at
15$\,\gevc$ incident beam momentum. The rates have to be scaled if the actual
time structure of the beam will be taken into account.
Figs.~\ref{fig:sim:Rate},\ref{fig:sim:FRate} show the single crystal rate for the
forward end cap and the barrel part for an energy threshold E$>$3$\,mev$.
Peak values of 60~kHz
and 500~kHz are reached in the most forward parts of the barrel and end cap,
respectively.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/rate_integral}
\caption[Single crystal rate for the forward end cap (and the barrel
section for an energy threshold of E$>$3~MeV using DPM at 15$\,\gevc$ incident
beam momentum. The barrel region is indicated by the ring numbers 1 to 72
(backward to forward angles). The forward end cap (green bars) is
sliced into 7 rings starting
from 20$^\circ$ to 5$^\circ$ in 2.5$^\circ$ degree steps (compare
Fig~\ref{fig:sim:FRate}).]
{Single crystal rate for the forward end cap (and the barrel
section for an energy threshold of E$>$3~MeV using DPM at 15$\,\gevc$ incident
beam momentum. The barrel region is indicated by the ring numbers 1 to 72
(backward to forward angles). The forward end cap (green bars) is
sliced into 7 rings starting
from 20$^\circ$ to 5$^\circ$ in 2.5$^\circ$ degree steps (compare
Fig~\ref{fig:sim:FRate}).}
\label{fig:sim:Rate}
\end{center}
\end{figure}


\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/forward_rate}
\caption[Single crystal rate for the forward end cap
for an energy threshold of E$>$3~MeV using DPM at 15$\,\gevc$ incident
beam momentum.]
{Single crystal rate for the forward end cap
for an energy threshold of E$>$3~MeV using DPM at 15$\,\gevc$ incident
beam momentum.}
\label{fig:sim:FRate}
\end{center}
\end{figure}

The energy differential single crystal hit rates are shown representatively in
Fig.~\ref{fig:sim:Ediff} for four different angles (5$^\circ$, 25$^\circ$,
 90$^\circ$ and 135$^\circ$).
The energy spectrum depends strongly on the polar angle and reflects the
kinematical enhancement of higher energies in forward direction. Moreover, the
large increase towards smaller energies originates from two effects. Firstly,
many charged particles traverse only a small fraction of a crystal. This
effect is amplified by
the non pointing geometry of the calorimeter. Secondly the large lateral
shower spread of $\gamma\slash e^{\pm}$ clusters converts into a large number
of hit
crystals, each with a small energy fraction.
 The summation of the given energy distributions
 yields the total absorbed energy rates of 27~mJ/h, 1.5~mJ/h, 0.16~mJ/h and
 0.03~mJ/h for each angle, respectively. The energy absorption is
 homogeneous in lateral direction of the crystals, but in radial direction the
 situation changes.
 The different
 interaction mechanisms of the passing particles with the
 scintillator material lead to an anisotropic energy deposition.
$\gamma\slash e^{\pm}$ deposit
a higher energy at the front faces of the crystals, whereas high energetic
(minimum ionizing) charged particles have a
 homogeneous energy distribution.
Only very slow (stopped) charged particles deposit more energy towards
the end face of the crystals (Bragg peak).
 It has to be taken into account, that $\gamma\slash e^{\pm}$ dominate the
 single crystal rate due to the much larger lateral shower size of the
 electromagnetic clusters.
  Fig~\ref{fig:sim:Erel} shows the simulated relative radial energy
 dose using the DPM cocktail of primary generated events at 15$\,\gevc$
 incident beam momentum. There is a strong variation of the relative energy
 absorption. The dose rates averaged over the full crystal of 25~mGy/h,
 1.4~mGy/h, 0.18~mGy/h and 0.03~mGy/h increase
 by a
 factor 2-3 in the first few cm of the front face of the crystals.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/energy_rate}
\caption[Single crystal energy differential rate spectrum for polar angles of
5$^\circ$ (black), 25$^\circ$ (blue),
 90$^\circ$ (red) and 135$^\circ$ (green) using DPM at 15$\,\gevc$ incident beam momentum.]
{Single crystal energy differential rate spectrum for polar angles of
5$^\circ$ (black), 25$^\circ$ (blue),
 90$^\circ$ (red) and 135$^\circ$ (green) using DPM at 15$\,\gevc$ incident beam momentum.}
\label{fig:sim:Ediff}
\end{center}
\end{figure}

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/reldose2}
\caption[Relative energy dose normalized to 1 as function of the
radial depth in a single crystal energy using DPM at 15$\,\gevc$ incident beam
momentum.]
{Relative energy dose normalized to 1 as function of the
radial depth in a single crystal energy using DPM at 15$\,\gevc$ incident beam
momentum.}
\label{fig:sim:Erel}
\end{center}
\end{figure}

Finally, the increase of the single crystal rate is studied, when instead of
an Hydrogen target a Carbon target is used. UrQMD has been used to generate
$\bar{p} ^{12}C \rightarrow X$ interactions.
Fig.~\ref{fig:sim:urqmd} shows
the single crystal rate ratio when Carbon as a solid target is
used. Both yields have been scaled to the same number of primary
interactions and are evaluated at 4$\,\gevc$ incident beam momentum.
 The absolute rate for $\bar{p} p \rightarrow X$ interactions
(DPM) at 4$\,\gevc$ is smaller by a factor of 2 compared 15$\,\gevc$.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/urqmd}
\caption[Single crystal rate ratio between UrQMD and DPM at 4~GeV incident beam
  momentum (description see \ref{fig:sim:Rate}).]
{Single crystal rate ratio between UrQMD and DPM at 4~GeV incident beam
  momentum (description see \ref{fig:sim:Rate}).
}
\label{fig:sim:urqmd}
\end{center}
\end{figure}



\section{APD Hit Rates}
The barrel part of the calorimeter is foreseen to be read out using avalanche
photodiodes (APD) as photo sensors. The leakage of ionization radiation from
primary
high energetic particles originating from the target and from decays
as well as secondary particles
created in the interactions with the detector material and support structures
lead to radiation damage of these sensors. This particle rates through the APDs
are estimated by a simulation
 using the Dual Parton Model (DPM) as generator for primary events.
The beam momentum of 15$\,\gevc$ has been used to evaluate the highest load for
$\bar{p} p \rightarrow X$ interactions. Detector individual APDs
 are implemented in the
full barrel section as Silicon material of 1$\times$2~cm$^2$ size and
40~$\mu$m thickness (corresponding to the sensitive APD layer).
A full tracking of the primary generated events through the whole
\Panda detector using GEANT4 was simulated.
The results are scaled
to the canonical interaction rate of 10$^7$ primary events/s.
Fig.~\ref{fig:sim:APDRate} shows the integral hit rate per APD
for the barrel section for
all traversing particles and specifically for protons and neutrons. The
particle cocktail
is composed mainly of 34\% pions, 19\% gammas, 19\% e$^\pm$, 16\% protons and
8\% neutrons.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/APD_rate}
\caption[Single APD rate for the barrel
section using DPM at 15$\,\gevc$ incident
beam momentum. The barrel region is indicated by the ring numbers 1 to 72
(backward to forward angles).]
{Single APD rate for the barrel
section using DPM at 15$\,\gevc$ incident
beam momentum. The barrel region is indicated by the ring numbers 1 to 72
(backward to forward angles).}
\label{fig:sim:APDRate}
\end{center}
\end{figure}

The single APD energy spectrum is
shown in Fig.~\ref{fig:sim:APDRateEdiff} for
the forward section of the barrel at 25$^\circ$.
The energy distribution for other angles is comparable.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/APD_rate_25deg}
\caption[Single APD energy differential rate for the barrel
section using DPM at 15$\,\gevc$ incident
beam momentum.]
{Single APD energy differential rate for the barrel
section using DPM at 15$\,\gevc$ incident
beam momentum.}
\label{fig:sim:APDRateEdiff}
\end{center}
\end{figure}





\section{Benchmark Studies}
As discussed in the introduction of this document the \Panda physics
program covers many fields and the addressed topics range from light
and charm hadron spectroscopy over study of charm in nuclear matter
and the measurement of the proton form-factors.  To fulfill the
requirements defined by the different fields the EMC is essential in
many cases. To demonstrate that the proposed \Panda detector and in
particular the EMC is able to reach the defined goals detailed Monte
Carlo studies have been performed. In the following the results of
these benchmark studies will be presented, where the EMC plays a
major role for the detection of the reactions defined as
benchmark. These studies cover charmonium spectroscopy as well as the
measurement of the time-like electromagnetic form-factors of the
proton. In the field of charmonium spectroscopy recent observations of
new states
\cite{bib:sim:newstates} falling in the mass range of the charmonium
system underline the importance of the ability to detect these states
in as many decay modes as possible to compare the observed decay
pattern with theoretical expectations and thus understand the nature of
these states. For the envisaged comprehensive study of the charmonium
system at \Panda this would imply the detection of hadronic, leptonic
and radiative decay modes, where the final states could consist out of
charged and neutral particles. Therefore photons have to be detected
with precise energy and spatial resolution over a wide energy range
and excellent coverage of the solid angle. For the reconstruction of
leptonic decays to
\ee (i.e., \jpsi and $\psi(2S)$ decays) the EMC supplements the PID
capabilities of the other detector components and provides together
with these a clean identification of electrons.  This is also crucial
for the measurement of the electromagnetic proton form factors in the
time-like region via the process $\pbarp\to\ee$, where the rejection
of the dominant $\pbarp \, \to \, \pip \, \pim$ background requires an excellent
separation of electrons and pions.


\subsection{$h_c$ detection with the $h_c \, \to \, \eta_{c} \, \gamma$ decay and the role of low energy $\gamma$-ray threshold} \label{sec:sim:h_c}
\subsubsection{Description of the studied channel}
$h_c$ is a singlet state of P wave charmonium ($1 ^{1}P_1$) with mass M=3526
MeV. One of its main decay modes is the electromagnetic transition to the
ground state, $\eta_c$, with the emission of a $\gamma$ with energy
$E_{\gamma}=503 MeV$. This decay mode was previously observed by E835
\cite{bib:sim:hc_E835} and CLEO experiments
\cite{bib:sim:hc_CLEO}. $h_c$ can be observed exclusively in many decay modes of
$\eta_c$, neutral ($\eta_c \, \to \, \gamma \, \gamma$) or
hadronic. The given analysis is based on $\eta_c \, \to \, \phi \,
\phi$ decay mode with $BR=2.6 \cdot 10^{-3}$ and $\phi$ decay
correspondingly $\phi \, \to \, K^{+} \, K^{-}, BR= 0.49$.

\subsubsection{Background consideration}
The previous observation of $h_c$ was done in neutral decay mode of $\eta_c$ in 
$\overline{p} p$ annihilation \cite{bib:sim:hc_E835} or in hadronic decay mode of $\eta_c$ from $e^{+} \, e^{-} \, \to \, \Psi(2S) \, \to \, \pi^{0} \, h_c, h_c \, \to \, \eta_c \, \gamma$ \cite{bib:sim:hc_CLEO}. In the case of 
PANDA experiment, where 
$h_c$ is produced in $\pbarp$ annihilation and detector is capable to study 
hadronic final states, the important aspect of analysis is the evaluation of signal to background 
ratio. This is due to the fact that production of the hadronic final states is much
more significant in $\pbarp$ annihilation in comparison with $e^{+}e^{-}$. 
For the exclusive decay mode considered in this study:
\begin{center}
$\pbarp \, \to \, h_c \, \to \, \eta_c \, \gamma \, \to \, \phi \, \phi \, \gamma \to K^{+} K^{-} K^{+} K^{-} \gamma$
\end{center}            
the following 3 reactions are considered as the main contributors to background:\\
\begin{enumerate}
\item
$\pbarp \to K^{+} K^{-} K^{+} K^{-} \pi^{0}$,
\item
$\pbarp \to \phi K^{+} K^{-} \pi^{0}$,
\item
$\pbarp \to \phi \phi \pi^{0}$.
\end{enumerate}
With one $\gamma$-ray left undetected from the $\pi^{0}$ decay these reactions have the same list of decay products as the studied $h_c$ decay.\\
In \Reffig{fig:sim:hc_e_gamma} the energy distributions of $\gamma$'s are 
presented for the signal and one of the background channels.

\begin{figure}
\begin{center}
\includegraphics[width=\swidth]{./sim/hc_e_gamma}
\caption[Energy distribution of the $\gamma$ for the $\pbarp \to h_c \to \eta_c \gamma$ and $\pbarp \to \phi \phi \pi^{0}$ reactions.]
{Energy distribution of the $\gamma$ for the $\pbarp \to h_c \to \eta_c \gamma$ and $\pbarp \to \phi \phi \pi^{0}$ reactions.}
\label{fig:sim:hc_e_gamma}
\end{center}
\end{figure}

The energy range of $\gamma$ from the $h_c$ decay is $[0.15; 2.0]\; \gev$. The 
corresponding distribution for the background on the one hand covers all this range and on
 the other hand has an increasing tendency towards zero energy. If we want to recover $\pi^{0}$ to separate signal from background, the low energy $\gamma$ reconstruction threshold should be as 
low as possible as it is discussed already in Section \ref{sec:sim:recothresh}. Moreover 
when one $\gamma$ from the $\pi^{0}$ has low energy, the other $\gamma$ together with 
charged hadrons has total momentum closer to the total momentum of the initial 
$\pbarp$ system. Such events pass cuts on the fit probability of the 4C-fit 
and this increases the relative importance of low energy threshold to apply anti-cut on
no $\pi^{0}$ in event and correspondingly to suppress background with $\pi^{0}$.

There are no experimental measurements, to our best knowledge, of the cross-sections for the studied background
reactions. The only way to estimate their cross-sections was found to use DPM 
(Dual Parton Model) event generator \cite{bib:sim:DPM}. $10^7$ events were generated with DPM at
beam momentum $p_z=5.609 \; \gevc$, which corresponds to the studied $h_c$ resonance. 
The corresponding numbers of events are 60 and 6 for the first two background channels. No events
for the $\pbarp \to \phi \phi \pi^{0}$ reaction were observed. With the
total $\pbarp$ cross-section at this beam momentum of $60 mb$ the cross-sections
for the corresponding background channels are estimated at 360 $nb$, 60 $nb$ and below
6 $nb$, respectively.

\subsubsection{Event selection}

The following selection criteria were applied to select the signal:
\begin{enumerate}
\item
constraint on a common vertex of $K^{+}$ and $K^{-}$ with $\phi$, pre-fit selection of 
$\eta_c$ invariant mass window [2.6;3.2] $\gev$ and $\phi$ mass window [0.8; 1.2] 
$\gev$,
\item
4C-fit to beam momentum, $CL> 0.05$,
\item
$\eta_c$ invariant mass [2.9;3.06] $\gev$,
\item
$E_{\gamma}$ within [0.4;0.6] $\gev$,
\item 
$\phi$ invariant mass [0.97;1.07] $\gev$,
\item
no $\pi^{0}$ candidates in event, i.e no 2 $\gamma$ invariant mass in the range 
[0.115;0.15] $\gev$ with 2 different low energy $\gamma$ threshold options: 30 $\mev$ 
and 10 $\mev$.
\end{enumerate}

\Reffig{fig:sim:hc_n_gamma} presents the multiplicity distribution of reconstructed EMC clusters for the signal and one of the background channels. One may note that the mean numbers of clusters, i.e. neutral candidates, significantly exceed one, expected for the signal, or two expected for the background from $\pi^{0}$ decay. This is caused by hadronic split-offs, which make it impossible to select as the signal events with only one cluster, because it leads to a significant drop of efficiency. This observation emphasizes the importance of other selection criteria, in particular of the anti-cut on no $\pi^{0}$ in an event. The latter strongly depends on the assumed low energy $\gamma$-ray threshold.

\begin{figure}
\begin{center}
\includegraphics[width=\swidth]{./sim/hc_n_gamma}
\caption[The number of reconstructed EMC clusters for the $\pbarp \to h_c \to \eta_c \gamma$ and $\pbarp \to \phi \phi \pi^{0}$ reactions.]
{The number of reconstructed EMC clusters for the $\pbarp \to h_c \to \eta_c \gamma$ and $\pbarp \to \phi \phi \pi^{0}$ reactions.}
\label{fig:sim:hc_n_gamma}
\end{center}
\end{figure}

\begin{table*}
\begin{center}
\begin{tabular}{|l|c|c|c|c|}
  \hline
  Selection criteria & signal & $4K \pi^{0}$ & $\phi  K^{+} K^{-} \pi^{0} $ & $\phi \phi \pi^{0}$ \\
    \hline
  pre-selection & 0.51 & $9.8\cdot 10^{-3}$ & $1.3\cdot 10^{-2}$ & $4.9\cdot 10^{-2}$\\
  $CL>0.05$ & 0.36 & $1.6\cdot 10^{-3}$ & $2.0\cdot 10^{-3}$ & $6.8\cdot 10^{-3}$\\
  $m(\eta_c), E_{\gamma}$ & 0.34 & $4.2\cdot 10^{-4}$ & $5.2\cdot 10^{-4}$ & $1.7\cdot 10^{-3}$ \\
  $m(\phi)$ & 0.33 & $1.0\cdot 10^{-5}$ & $1.2\cdot 10^{-4}$ & $1.7\cdot 10^{-3}$ \\
  $no \; \pi^{0} (30 MeV)$ & 0.27 & $1.0\cdot 10^{-5}$ & $4.5\cdot 10^{-5}$ & $8.6\cdot 10^{-4}$ \\
  $no \; \pi^{0} (10 MeV)$ & 0.25 & $5.0\cdot 10^{-6}$ & $3.0\cdot 10^{-5}$ & $7.0\cdot 10^{-4}$ \\

  \hline
\end{tabular}
\caption[Efficiency of different event selection criteria]{Efficiency of different event selection criteria}             
\label{tab:perf:hc_eff}
\end{center}
\end{table*}

\begin{table}
\begin{center}
\begin{tabular}{|l|c|}
  \hline
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  channel & Signal/background ratio\\
    \hline
  $\pbarp \to K^{+} K^{-} K^{+} K^{-} \pi^{0}$ & 3.5 \\
  $\pbarp \to \phi K^{+} K^{-} \pi^{0}$ & 10\\
  $\pbarp \to \phi \phi \pi^{0}$ & $>6$\\
  \hline
\end{tabular}
\caption[Signal to background ratio for different $h_c$ background channels]{Signal to background ratio for different $h_c$ background channels}          
\label{tab:perf:hc_sb_ratio}
\end{center}
\end{table}

\subsubsection{Signal to background ratio vs low energy $\gamma$-ray threshold}
The efficiency of the corresponding selection criteria is given in \Reftbl{tab:perf:hc_eff} for the signal and the considered background channels.

Assuming the $h_c$ production cross-section of $40 nb$, one gets signal to background
ratio as given in \Reftbl{tab:perf:hc_sb_ratio}.

For the $\pbarp \to \phi \phi \pi^{0}$ background channel the 
reduction of low energy $\gamma$-ray threshold from 30 MeV to 10 MeV gives $20\percent$ improvement in the signal to background ratio, for the
$\pbarp \to \phi K^{+} K^{-} \pi^{0}$ corresponding improvement is $40\percent$.

With the final signal selection efficiency of $25\percent$ and the assumed luminosity of
$L=10^{32}\cm^{-2}s^{-1}$ the expected signal event rate is 55 events/day.\\

\subsection{$Y(4260)$ in formation}
The recently discovered vector-state $Y(4260)$, having a mass and
width of 4259 \mevcc and 88\mev, respectively is observed only in the
$\jpsi\pi\pi$ decay mode. Here the reaction $Y(4260)\to\jpsi\piz\piz$
is studied in
\pbarp-formation and the decay chain is exclusively reconstructed via 
$\jpsi\to\ee$ and $\piz\to\gamma\gamma$.

Electron candidates are identified by the global likelihood selection
algorithm described above. For the reconstruction of $\jpsi\to\ee$
decays at least one of the lepton candidates must have a likelihood
value $L>0.99$ while the other candidate should fulfill $L>0.85$. The
corresponding tracks of the $\ee$ candidates are fitted to a common
vertex and an accepted candidate should have a confidence level of
$CL>0.1\%$. Photon candidates are formed from the clusters found in
the EMC applying the reconstruction algorithm described above, must
have an energy $>200\mev$ and are combined to $\piz\to\gamma\gamma$
candidates.

Accepted \jpsi and \piz candidates are combined to $\jpsi\piz\piz$
candidates, where the \piz candidates should not share the same photon
candidate. The final state lepton and photon candidates are
kinematically fitted by constraining the sums of their spatial
momentum components and energies to the corresponding values of the
initial \pbarp system. An accepted $\jpsi\piz\piz$ candidate must have
a confidence level of $CL>0.1\%$ and the invariant mass of the \ee and
$\gamma\gamma$ subsystems should be within $[3.07;3.12]\gevcc$ and
$[120;150]\mevcc$, respectively. A FWHM of $\approx 14\mevcc$
($\approx 7\mevcc$) is obtained for the \jpsi (\piz) signal after the
kinematic fit (\Reffig{fig:sim:jpsipipi}). For the final event
selection $\jpsi\piz\piz$ candidates are refitted kinematically by
constraining the invariant
\ee mass to the
\jpsi mass and the invariant $\gamma\gamma$ mass to the \piz mass on
top of the constraints applied to the initial
\pbarp four-vector. Only events where exactly one valid $\jpsi\piz\piz$ candidate
with $CL>0.1\%$ is found are accepted for further analysis.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/jpsipipi}
\caption[Invariant $\jpsi\to\ee$ and $\piz\to\gamma\gamma$ mass for the process $\ppbar\to Y(4260)\to\jpsi\piz\piz$]
{Invariant a) $\jpsi\to\ee$ and b) $\piz\to\gamma\gamma$ mass after
the kinematic fit with constraints on the initial \pbarp system as
described in the text. The vertical lines indicate the mass windows
chosen for further selection.}
\label{fig:sim:jpsipipi}
\end{center}
\end{figure}

To reject background from the reactions $\pbarp\to\jpsi\eta\eta$
($\pbarp\to\jpsi\eta\piz$) with $\eta\to\gamma\gamma$ the events are
reconstructed and kinematically fitted similar to the fit with the
$\jpsi\piz\piz$ signal hypothesis described above but assuming the
$\jpsi\eta\eta$ ($\jpsi\eta\piz$) hypothesis, where $\eta$ candidates
should have an invariant mass within $[500;600]\mevcc$. Events where
at least one valid $\jpsi\eta\piz$ or $\jpsi\eta\eta$ candidate with
$CL>0.01\%$ is found are rejected.

The reconstruction efficiency after all selection criteria is found to
be $13.8$\%. For $\pbarp\to\jpsi\eta\eta$ and $\pbarp\to\jpsi\eta\piz$
events the suppression rate is better than $10^4$ and the
contamination of the $\jpsi\piz\piz$ signal with events from these
reactions is expected to be negligible unless the cross sections for
$\pbarp\to\jpsi\eta\eta$ and $\pbarp\to\jpsi\eta\piz$ are enhanced by
more than an order of magnitude compared to the signal cross
section. Another source of background which has been investigated are
non-resonant $\pbarp\to\pip\pim\piz\piz$ events. For this reaction an
upper limit of $132\mubarn$ at 90\% CL can be derived from the
measurement at $\sqrt{s}=4.351\gevcc$ \cite{bib:sim:XXX}, $92\mevcc$
above the $Y(4260)$ resonance. The cross section for the signal
reaction is estimated from Ref.~\cite{bib:sim:XXX} to be in the order
of $50\pb$. This requires a suppression for
$\pbarp\to\pip\pim\piz\piz$ of at least $10^7$, whereas with the
currently available amount of MC events a suppression better than
$10^7$ is obtained.

In summary the reconstruction of the $Y(4260)\to\jpsi\piz\piz$ decay
mode with one \ee pair and four photons in the final state yields a
good detection efficiency and suppression of the dominant
$\pbarp\to\pip\pim\piz\piz$ background.

\subsection{Charmonium Hybrid in Production}
Closely connected with charmonium spectroscopy is the search for
predicted exotic hadrons with hidden charm, such as charmonium
molecule, tetra-quark or hybrid states. For the latter the ground
state is generally expected to be a spin-exotic $J^{PC}=1^{-+}$ state
and lattice QCD calculations predict its mass in the range between
$4100$ and $4400\mevcc$. In \pbarp annihilation this state can be
produced only in association with one or more recoiling particles. Here
the results of a study assuming the production of a state having a
mass $4290\mevcc$ and a width of $20\mev$ together with a $\eta$ meson
are reported.

Flux-tube model calculations predict for a hybrid state of this mass
suppressed decays to open charm with respect to hidden charm
decays. An OZI-allowed decay to hidden charm would be the transition
to $\chi_{c1}$ with emission of light hadrons, preferable scalar
particles. The lightest scalar system is composed out of two neutral
pions in a relative $s$-wave.

In the study the decay of the charmonium hybrid (labeled as $\psi_g$ in
the following) to $\chi_{c1}(\piz\piz)_s$ with the subsequent
radiative $\chi_{c1}\to\jpsi\gamma$ decay with $\jpsi$ decaying to a
lepton pair \ee or \mumu is considered. The recoiling meson is
reconstructed from the decay $\eta\to\gamma\gamma$. The total
branching fraction for the subsequent $\psi_g$ and $\eta$ decays is
given by $\mathcal{B}(\psi_g\to\chi_{c1}\piz\pi)\times 1.6\%$, where
$\mathcal{B}(\psi_g\to\chi_{c1}\piz\pi)$ is the unknown branching
fraction of the $\psi_g$ decay.

Photon candidates are selected from the clusters found in the EMC with
the reconstruction algorithm described in \ref{XXX}. Two photon
candidates are combined and accepted as \piz and $\eta$ candidates if
their invariant mass is within the interval [115;150]\mevcc and
[470;610]\mevcc, respectively.

For the reconstruction of \jpsi decays two candidates of opposite
charge, both identified as electrons or muons applying the likelihood
selection algorithm described in \ref{XXX} and having a likelihood
value $L>0.2$ are combined and accepted as \jpsi candidates if their
invariant mass is within the interval $[2.98;3.16]\gevcc$. The
corresponding tracks of the two lepton candidates are kinematically
and geometrically fitted to a common vertex and constraining their
invariant mass to the nominal \jpsi mass. 

Afterwards $\chi_{c1}\to\jpsi\gamma$ candidates are formed by
combining accepted
\jpsi and photon candidates, whose invariant mass is within the range $3.3$-$3.7$\gevcc.
From these $\chi_{c1}\piz\piz\eta$ candidates are created, where the
same photon candidate does not occur more than once in the final
state.  The corresponding tracks and photon candidates of the final
state are kinematically fitted by constraining their momentum and
energy sum to the initial \pbarp system and the invariant lepton
candidates mass to the \jpsi mass. Accepted candidates must have a
confidence level of $CL>0.1\%$ and the invariant mass of the
$\jpsi\gamma$ subsystem should be within the range
$[3.49;3.53]\gevcc$, whereas the invariant mass of the $\eta$
candidates must be within the interval $[530;565]\mevcc$. A FWHM of
$\approx 13\mevcc$ is observed for the $\chi_{c1}$ and $\eta$ signals
(\Reffig{fig:sim:hybridChiEta}) after the kinematic fit.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/hybridChiEta}
\caption[Invariant $\chi_{c1}\to\jpsi\gamma$ and $\eta\to\gamma\gamma$ mass for the process $\ppbar\to \psi_g\eta$]
{Invariant a) $\chi_{c1}\to\jpsi\gamma$ and b) $\eta\to\gamma\gamma$
mass after the kinematic fit with constraints on the initial \pbarp
system as described in the text. The vertical lines indicate the mass
windows chosen for further selection.}
\label{fig:sim:hybridChiEta}
\end{center}
\end{figure}


For the final event selection the same kinematic fit is repeated with
additionally constraining the invariant $\chi_{c1}$, \piz and $\eta$
invariant mass to the corresponding nominal mass values. Candidates
having a confidence level less than $0.1\%$ are rejected. If more than
one candidate is found in an event, the candidate with the biggest
confidence level is chosen for further analysis. Thus events with a
$\jpsi$ candidate reconstructed from the decay to \ee or \mumu are
unambiguously disentangled. It has been found that no event with a
$\jpsi\to\ee$ decay was misidentified as a $\jpsi\to\mumu$ and vice
versa.

The reconstruction efficiency after all selection criteria is $4.2\%$
and $5.8\%$ for events with $\jpsi\to\ee$ and $\jpsi\to\mumu$ decays,
respectively. The invariant $\chi_{c1}\piz\piz$ mass is shown in
\Reffig{fig:sim:hybrid}. The $\psi_g$ signal has a FWHM of $27\mevcc$.


\begin{figure}[htb]
\begin{center}
\includegraphics[width=\swidth]{./sim/hybrid}
\caption[Invariant $\chi_{c1}\piz\piz$ mass for the reaction $\ppbar\to \psi_g\eta$]
{Invariant $\chi_{c1}\piz\piz$ mass after the kinematic fit with
constraints on the initial \pbarp system and resonances as described
in the text.}
\label{fig:sim:hybrid}
\end{center}
\end{figure}

The final state with 7 photons and a \ee or \mumu lepton pair
originating from \jpsi decays has a distinctive signature and
separation from light hadron background should be feasible.  
Another source of background are events with hidden charm, in
particular events including a \jpsi meson. This type of background has
been studied by analyzing $\pbarp\to\chi_{c0}\piz\piz\eta$,
$\pbarp\to\chi_{c1}\piz\eta\eta$ and
$\pbarp\to\chi_{c1}\piz\piz\piz\eta$. The hypothetical hybrid state is
absent in these reactions, but the $\chi_{c0}$ and $\chi_{c1}$ mesons
decay via the same decay path as for signal. Therefore these events
have a similar topology as signal events and could potentially pollute
the $\psi_g$ signal. The suppression after application of all
selection criteria is found to be $7\cdot 10^3$
($\pbarp\to\chi_{c0}\piz\piz\eta$), $3\cdot 10^4$
($\pbarp\to\chi_{c1}\piz\eta\eta$) and $1\cdot 10^5$
($\pbarp\to\chi_{c1}\piz\piz\piz\eta$). Therefore low contamination of
the $\psi_g$ signal from this background reactions is expected.


\subsection{Time-like electromagnetic form-factors}
The electric ($G_E$) and magnetic ($G_M$) form factor of the proton
parameterize the hadronic current in the matrix element for elastic
electron scattering $\ee\to\pbarp$ and in its crossed process
$\pbarp\to\ee$ annihilation. The form-factors are analytic functions
of the four momentum transfer $q^2$ ranging from $q^2=-\inf$ to
$q^2=+inf$. The annihilation process allows to access positive $q^2$
(time like) starting from the threshold of $q^2 = 4 m_p^2$. In this
region $G_E$ and $G_M$ become complex functions and their
determination for low to intermediate momentum transfer is an open
question. At \Panda this region can be accessed between $5(\gevc)^2$
and $22(\gevc)^2$. The differential cross section for the reaction
$\pbarp\to\ee$ is given by
\begin{eqnarray}
\frac{\mathrm{d}\sigma}{\mathrm{d}\cos\theta}&=&\frac{\pi\alpha^2}{8m_p^2\sqrt{\tau\left(\tau-1\right)}} \nonumber  \\
 & &   \Huge(|G_M|^2 \left (1+\cos^2 \theta \right ) \nonumber\\
& + &\frac{|G_E|^2}{\tau} \left( 1-\cos^2 \theta \right ) \Huge) 
\end{eqnarray}
where $\tau=s/4m^2_p$. The factors $|G_E|$ and $|G_M|$ can be
determined from the angular distribution of $\pbarp\to\ee$ events in
dependence of the beam momentum. A measurement of the luminosity will
provide a measurement of both factors $|G_E|$ and $|G_M|$, otherwise
the absolute height of the cross section remains unknown and only the
ratio $|G_E|/|G_M|$ is accessible. However, for a precise
determination of the form factors a suppression better than $10^8$ of
the dominant background from $\pbarp\to\pip\pim$, having a cross
section about $10^6$ times higher than the signal reaction is
mandatory.

To achieve the required background suppression a good separation of
electrons and pions over a wide momentum range up to $\approx 15\gevc$
is mandatory, where the PID information from the individual detector
components has to be exploited. In particular information from the EMC
is important in the high momentum range where PID measurements from
the tracking, Cherenkov and muon detectors do not allow to distinguish
between the two species.

For the reconstruction of $\pbarp\to\ee$ two candidates identified as
electrons having a likelihood value $>0.998$ are combined. The two
tracks are kinematically fitted by constraining the sum of the
four-momenta to the four-momentum of the initial \pbarp system and are
accepted as a \ee candidate if the fit yields a confidence level
greater than $1\%$.  The same fit is repeated but assuming pion
hypothesis for the two tracks. If this fit yields a CL which is larger
than 10 times the one obtained for the electron hypothesis the
corresponding candidate is rejected. For events where more than one
valid \ee candidate is found, only the candidate with the biggest
confidence level is considered for further analysis.

For the measurement of $|G_E|$ and $|G_M|$ the angle $\theta$ between
the $e^+$ candidate's direction of flight and the beam axis is
computed in the center of mass system. The obtained $\cos(\theta)$
distribution is corrected by the $\cos(\theta)$-dependent
reconstruction efficiency. In lack of an absolute luminosity
measurement for MC data only the ratio $|G_E|/|G_M|$ can be determined
from a fit to the corrected $\cos(\theta)$ distribution. In
\Reffig{fig:sim:epemang} the corrected distribution for
$\sqrt{s}=3.3\gevc$ is shown exemplarily, whereas a ratio
$|G_E|/|G_M|$ of 0 and $3$ has been assumed in the simulation. The
values $0\pm 0.17$ and $3.01\pm 0.13$ derived from the fit are in full
agreement with the input values of the simulation.

\begin{figure}[tb]
\begin{center}
\includegraphics[width=\swidth]{./sim/epemCosTheta.png}
\caption[Angular distribution of reconstructed $\pbarp\to\ee$ events.]
{Angular distribution for reconstructed $\pbarp\to\ee$ events at an
incident beam momentum of $3.3\gevc$ after efficiency correction. For
the ratio of the form-factors $|G_E|/|G_M|$ a value of $0$ (blue) and
$3$ (red) has been assumed in the simulation. The functions overlaid
to the data points correspond to the result of the fit described in
the text.}
\label{fig:sim:epemang}
\end{center}
\end{figure}

With the currently available amount of MC events the background
rejection of $\pbarp\to\pip\pim$ is found to be better than $10^7$.
Studies including larger amount of background data and different beam
momenta ranging from 1.5-15\gevc are presently ongoing.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "/windows/D/EmcTdr/v13/PndEmcTdr/Tex/lit_emc.bib"
%%% End: 


==> sty/panda_commands.tex <==
% def_panda_cmd.tex
%
\RequirePackage[centertags]{amsmath}
%
\RequirePackage{xspace}
%\RequirePackage{ulem}
%
\def\MARK#1{\texorpdfstring{{\emph{\textcolor{red}{#1}}}}{{#1}}}
%\def\MARK#1{\emph{\textcolor{red}{#1}}}
%\def\MARK#1{{\bf \textcolor{red}{#1}}}
%\def\MARK#1{{#1}}
% use to mark text 
% (Text will be kept, but the marking removed in the final document)
%
\def\COM#1{\fbox{\parbox{\swidth}{\textcolor{red}{\bf COMMENT: #1}}}}
%\def\COM#1{}
% use to add comments
% (The whole will be removed in the final version)
%
% use to mark parts, which shouldn't be present in the cost-free version

\def\OnlyLayoutColumnBreak{{\vfill\newpage}}%

\def\OnlyLayoutPageBreak{{\vfill\clearpage}}%

\def\OnlyLayoutDoublePageBreak{{\vfill\cleardoublepage}}%

%
\def\bfg{\begin{figure}}%
\def\efg{\end{figure}}%
\def\bc{\begin{center}}%
\def\ec{\end{center}}%
\def\bi{\begin{itemize}}%
\def\ei{\end{itemize}}%
\def\be{\begin{equation}}%
\def\ee{\end{equation}}%
\def\bn{\begin{eqnarray}}%
\def\en{\end{eqnarray}}%
\def\ba#1{\left(\begin{array}{#1}}%
\def\ea{\end{array}\right)}%
\def\bef{\begin{equation}\fbox{$\displaystyle}%
\def\eef{$}\end{equation}}%
\def\bnf{\bef\ba{rcl}}%
\def\enf{\ea\eef}%
%\def\refeq#1{\Eqref{#1}\xspace}%
%\def\Refsec#1{sec.~\ref{#1}\xspace}%
%\def\Refchap#1{\Refchap{#1}\xspace}%
%\def\Reffig#1{\Reffig{#1}\xspace}%
%\def\Reftbl#1{\Reftbl{#1}\xspace}%
%\def\reftab#1{\Reftbl{#1}\xspace}%
\def\Refeq#1{Eq.~\ref{#1}\xspace}%
\def\Refeqs#1{Eqs.~\ref{#1}\xspace}%
\def\Refsec#1{Sec.~\ref{#1}\xspace}%
\def\Refchap#1{Chap.~\ref{#1}\xspace}%
\def\Reffig#1{Fig.~\ref{#1}\xspace}%
\def\Reffigs#1{Figs.~\ref{#1}\xspace}%
\def\Reftbl#1{Table~\ref{#1}\xspace}%
\def\Reftbls#1{Tables~\ref{#1}\xspace}%
\def\RefeqX#1{Eq.~\ref{#1}}%
\def\RefeqsX#1{Eqs.~\ref{#1}}%
\def\RefsecX#1{Sec.~\ref{#1}}%
\def\RefchapX#1{Chap.~\ref{#1}}%
\def\ReffigX#1{Fig.~\ref{#1}}%
\def\ReffigsX#1{Figs.~\ref{#1}}%
\def\ReftblX#1{Table~\ref{#1}}%
\def\ReftblsX#1{Tables~\ref{#1}}%
%\def\Reftab#1{Table~\ref{#1}\xspace}%
\def\ub{\underbrace}%
%
\def\vps{\hspace*{5mm}}%
\def\dsty{\displaystyle}%
%
\newcounter{auth}%
\setcounter{auth}{0}%
\def\authitem#1{\addtocounter{auth}{1}#1}%
\def\authitemi#1#2{\addtocounter{auth}{1}#2$^{#1}$}%
\newcounter{inst}%
\setcounter{inst}{0}%
\def\institem#1{\par \addtocounter{inst}{1}#1\\}%
\def\lastitem{\ }%
\def\respitem#1{\institem{{\bf #1}\lastitem\\}}%
\let\groupitem=\authitem
%
\newcommand{\captionfonts}{\small}
%
\makeatletter  % Allow the use of @ in command names
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  \sbox\@tempboxa{{\captionfonts {\bf #1:} #2}}%
  \ifdim \wd\@tempboxa >\hsize
    {\captionfonts {\bf #1:} #2\par}
  \else
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
\makeatother   % Cancel the effect of \makeatletter
%
% a few commands to change the figure placing (commented are the default values)
%\renewcommand{\textfraction}{0.1} % 0.2
%\renewcommand{\bottomfraction}{0.4} % 0.3
%\renewcommand{\dbltopfraction}{0.8} % 0.7
%\renewcommand{\dblfloatpagefraction}{0.3} % 0.5
%\renewcommand{\floatpagefraction}{0.3} % 0.5
%\setcounter{dbltopnumber}{3} % 2
%\setcounter{bottomnumber}{2} % 1
%
\def\markpanda#1#2{\markboth{\Panda{} - #1}{FAIR/PANDA/#2}}%
%
% EOF: def_panda_cmd.tex


==> sty/panda_detector.tex <==
% panda_detector.tex
%
\RequirePackage{xspace}
%
\def\INST#1{\texorpdfstring{{\sf #1}}{{#1}}\xspace}%
%
\def\PANDA{\texorpdfstring{$\overline{\mbox{\sf P}}${\sf ANDA}}{Panda}\xspace}%
\def\Panda{\texorpdfstring{$\overline{\mbox{\sf P}}${\sf ANDA}}{Panda}\xspace}%
\def\HESR{\INST{HESR}}%
\def\Hesr{\INST{HESR}}%
\def\GSI{\INST{GSI}}%
\def\Gsi{\INST{GSI}}%
\def\FAIR{\INST{FAIR}}%
\def\Fair{\INST{FAIR}}%
%
\def\Ts{TS\xspace}
\def\Fs{FS\xspace}
\def\Mvd{MVD\xspace}
%\def\Emc{EMC\xspace}
%\def\TsEmc{TS-EMC\xspace}
%\def\FsEmc{FS-EMC\xspace}
\def\Had{HAD\xspace}
\def\Muo{MUO\xspace}
\def\TsMuo{TS-MUO\xspace}
\def\FsMuo{FS-MUO\xspace}
\def\Stt{STT\xspace}
\def\Tpc{TPC\xspace}
\def\Dirc{DIRC\xspace}
\def\Rich{RICH\xspace}
\def\Mdc{MDC\xspace}
\def\TsMdc{TS-MDC\xspace}
\def\FsMdc{FS-MDC\xspace}
\def\Tof{TOF\xspace}
\def\Lum{LUM\xspace}
\def\Mag{MAG\xspace}
\def\TsMag{SOL\xspace}
\def\FsMag{DIP\xspace}
%
% EMC definitions
\def\Emc{EMC\xspace}
\def\BEMC{barrel EMC\xspace}
\def\FWEMC{forward endcap EMC\xspace}
\def\BWEMC{backward endcap EMC\xspace}
\def\TSEMC{target spectrometer EMC\xspace}
\def\FSEMC{forward spectrometer EMC\xspace}
\def\TsEmc{\TSEMC}
\def\FsEmc{\FSEMC}
%
\def\LAAPD{LAAPD\xspace}
\def\LAAPDs{LAAPDs\xspace}
\def\VPT{VPT\xspace}
\def\VPTs{VPTs\xspace}
\def\PWOII{PWO-II\xspace}
\def\PWO{PWO\xspace}
%
% EOF: def_panda_det.tex


==> sty/panda_symbols.tex <==
% def_panda_sym.tex
%
\input{./sty/pennames.sty}
\input{./sty/myunits.sty}
\input{./sty/mymath.sty}
%
\RequirePackage{xspace}
% Upright mu for micro
\DeclareFontFamily{U}{euc}{}% I chose euc because the chart is called Euler cursive
\DeclareFontShape{U}{euc}{m}{n}{<-6>eurm5<6-8>eurm7<8->eurm10}{}%
\DeclareSymbolFont{AMSc}{U}{euc}{m}{n} % I chose AMSc because AMSa and AMSb are defined in the amsfonts-package
\DeclareMathSymbol{\umu}{\mathord}{AMSc}{"16}
%
%
\def\degrees{\ensuremath{^\circ}\xspace}%
\def\percent{$\,$\%\xspace}%
\def\prm{\ensuremath{^\prime}}%
\def\etc{{\em etc.}\xspace}%
%
\def\tm{\texttrademark}
\def\tmr{\ensuremath{^{\textregistered}}}
%
\def\ppbar{\ensuremath{\mbox{p}\overline{\mbox{p}}}\xspace}%
\def\pbarp{\ensuremath{\overline{\mbox{p}}\mbox{p}}\xspace}%
\def\pbarA{\ensuremath{\overline{\mbox{p}}\mbox{A}}\xspace}%
\def\pbarN{\ensuremath{\overline{\mbox{p}}\mbox{N}}\xspace}%
\def\pbard{\ensuremath{\overline{\mbox{p}}\mbox{d}}\xspace}%
\def\pbar{\ensuremath{\overline{\mbox{p}}}\xspace}%
\def\nbar{\ensuremath{\overline{\mbox{n}}}\xspace}%
\def\pbarn{\ensuremath{\overline{\mbox{p}}\mbox{n}}\xspace}%
\def\nbarn{\ensuremath{\overline{\mbox{n}}\mbox{n}}\xspace}%
%
\def\qbar{\ensuremath{\overline{q}}\xspace}%
\def\cbar{\ensuremath{\overline{c}}\xspace}%
\def\ccbar{\ensuremath{c\overline{c}}\xspace}%
\def\ccbarg{\ensuremath{c\overline{c}g}\xspace}%
\def\cqbar{\ensuremath{c\overline{q}}\xspace}%
\def\cbarq{\ensuremath{\overline{c}q}\xspace}%
\def\uubar{\ensuremath{u\overline{u}}\xspace}%
\def\ddbar{\ensuremath{d\overline{d}}\xspace}%
\def\ssbar{\ensuremath{s\overline{s}}\xspace}%
\def\bbbar{\ensuremath{b\overline{b}}\xspace}%
\def\bqbar{\ensuremath{b\overline{q}}\xspace}%
\def\bbarq{\ensuremath{\overline{b}q}\xspace}%
\def\qqbar{\ensuremath{q\overline{q}}\xspace}%
\def\qqbarg{\ensuremath{q\overline{q}g}\xspace}%
\def\QQbar{\ensuremath{Q\overline{Q}}\xspace}%
%
\def\ee{\ensuremath{e^+e^-}\xspace}%
\def\mumu{\ensuremath{\mu^+\mu^-}\xspace}%
%
\def\piz{\ensuremath{\pi^0}\xspace}%
\def\pip{\ensuremath{\pi^+}\xspace}%
\def\pim{\ensuremath{\pi^-}\xspace}%
\def\pipm{\ensuremath{\pi^\pm}\xspace}%
\def\pimp{\ensuremath{\pi^\mp}\xspace}%
%
\def\K{\ensuremath{K}\xspace}%
\def\Kp{\ensuremath{K^+}\xspace}%
\def\Km{\ensuremath{K^-}\xspace}%
\def\Kpm{\ensuremath{K^\pm}\xspace}%
\def\Kmp{\ensuremath{K^\mp}\xspace}%
\def\KKbar{\ensuremath{K\overline{K}}\xspace}%
\def\Kz{\ensuremath{K^0}\xspace}%
\def\Kzbar{\ensuremath{\overline{K}^0}\xspace}%
\def\KzKzbar{\ensuremath{K^0\overline{K^0}}\xspace}%
\def\Ks{\ensuremath{K_S^0}\xspace}%
\def\Kl{\ensuremath{K_L^0}\xspace}%
%
\def\etaprime{\ensuremath{\eta\prm}\xspace}%
\def\pione{\ensuremath{\pi_1}\xspace}%
%
\def\uquark{\ensuremath{u}\xspace}%
\def\dquark{\ensuremath{d}\xspace}%
\def\squark{\ensuremath{s}\xspace}%
\def\cquark{\ensuremath{c}\xspace}%
\def\bquark{\ensuremath{b}\xspace}%
\def\tquark{\ensuremath{t}\xspace}%
%
\def\D{\ensuremath{D}\xspace}%
\def\Dbar{\ensuremath{\overline{D}}\xspace}%
\def\DDbar{\ensuremath{D\overline{D}}\xspace}%
\def\DpDm{\ensuremath{D^+D^-}\xspace}%
\def\Dz{\ensuremath{D^0}\xspace}%
\def\Dzbar{\ensuremath{\overline{D}^0}\xspace}%
\def\DzDzbar{\ensuremath{D^0\overline{D}^0}\xspace}%
\def\Dx{\ensuremath{D^\ast}\xspace}%
\def\Dxbar{\ensuremath{\overline{D}^\ast}\xspace}%
\def\DxDxbar{\ensuremath{D^\ast\overline{D}^\ast}\xspace}%
\def\Dxz{\ensuremath{D^{\ast 0}}\xspace}%
\def\Dxzbar{\ensuremath{\overline{D}^{\ast 0}}\xspace}%
\def\DbarDxx{\ensuremath{D\overline{D}^{\ast\ast}}\xspace}%
%
\def\Ds{\ensuremath{D_s}\xspace}%
\def\Dspm{\ensuremath{D_s^\pm}\xspace}%
\def\Dsmp{\ensuremath{D_s^\mp}\xspace}%
\def\Dsx{\ensuremath{D_s^\ast}\xspace}%
\def\Dsxpm{\ensuremath{D_s^{\ast\pm}}\xspace}%
\def\Dsxmp{\ensuremath{D_s^{\ast\mp}}\xspace}%
\def\DsDsbar{\ensuremath{D_s\overline{D_s}}\xspace}%
\def\DspDsm{\ensuremath{D_s^+D_s^-}\xspace}%
\def\DsxDsxbar{\ensuremath{D_s^\ast\overline{D_s}^\ast}\xspace}%
\def\DsbarDsxx{\ensuremath{\overline{D_s}D_s^{\ast\ast}}\xspace}%
%
\def\jpsi{\ensuremath{J\!/\!\psi}\xspace}%
\def\psiprime{\ensuremath{\psi\prm}\xspace}%
\def\etac{\ensuremath{\eta_c}\xspace}%
\def\etacprime{\ensuremath{\eta\prm_c}\xspace}%
\def\chicJ{\ensuremath{\chi_{cJ}}\xspace}%
\def\chiczero{\ensuremath{\chi_{c0}}\xspace}%
\def\chicone{\ensuremath{\chi_{c1}}\xspace}%
\def\chictwo{{\chi_{c2}}\xspace}%
\def\honec{\ensuremath{h_c}\xspace}%
%
\def\Cascade{\ensuremath{\Xi}\xspace}%
\def\Cascadebar{\ensuremath{\overline{\Xi}}\xspace}%
\def\LambdaLambdabar{\ensuremath{\Lambda\overline{\Lambda}}\xspace}%
\def\OmegaOmegabar{\ensuremath{\Omega\overline{\Omega}}\xspace}%
\def\SigmaSigmabar{\ensuremath{\Sigma\overline{\Sigma}}\xspace}%
\def\CascadeCascadebar{\ensuremath{\Xi\overline{\Xi}}\xspace}%
%
\def\kev{{\mbox{keV}}\xspace}%
\def\kevcc{{\mbox{keV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\mev{{\mbox{MeV}}\xspace}%
\def\mevc{{\mbox{MeV}\!/\!\mbox{\em c}}\xspace}%
\def\mevcc{{\mbox{MeV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\mevccsq{{\mbox{MeV$^2$}\!/\!\mbox{\em c$^4$}}\xspace}%
\def\gev{{\mbox{GeV}}\xspace}%
\def\gevc{{\mbox{GeV}\!/\!\mbox{\em c}}\xspace}%
\def\gevcsq{{\mbox{GeV$^2$}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\gevcc{{\mbox{GeV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\gevccsq{{\mbox{GeV$^2$}\!/\!\mbox{\em c$^4$}}\xspace}%
%
\def\aC{{\mbox{aC}}\xspace}%
%
\def\barn{\ensuremath{\rm \,b}\xspace}
\def\barnhyph{\ensuremath{\rm -b}\xspace}
\def\mbarn{\ensuremath{\rm \,mb}\xspace}
\def\mbarnhyph{\ensuremath{\rm -mb}\xspace}
\def\mubarn{\ensuremath{\rm \,\mu b}\xspace}
\def\nb{\ensuremath{\rm \,nb}\xspace}
\def\pb {\ensuremath{\rm \,pb}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
%
\def\JPC{\ensuremath{J^{\!P\!C}}\xspace}%
\def\JPCzeropm{\ensuremath{0^{+-}}\xspace}%
\def\JPCzeropp{\ensuremath{0^{++}}\xspace}%
\def\JPCzeromm{\ensuremath{0^{--}}\xspace}%
\def\JPCzeromp{\ensuremath{0^{-+}}\xspace}%
\def\JPConepm{\ensuremath{1^{+-}}\xspace}%
\def\JPConepp{\ensuremath{1^{++}}\xspace}%
\def\JPConemm{\ensuremath{1^{--}}\xspace}%
\def\JPConemp{\ensuremath{1^{-+}}\xspace}%
\def\JPCtwopm{\ensuremath{2^{+-}}\xspace}%
\def\JPCtwopp{\ensuremath{2^{++}}\xspace}%
\def\JPCtwomm{\ensuremath{2^{--}}\xspace}%
\def\JPCtwomp{\ensuremath{2^{-+}}\xspace}%
%
\def\JPCscalar{\JPCzeropp}%
\def\JPCvector{\JPConemm}%
\def\JPCtensor{\JPCtwopp}%
%
\def\extl{\ensuremath{E_{xtl}}\xspace}
\def\ecl{\ensuremath{E_{cl}}\xspace}
\def\emax{\ensuremath{E_{max}}\xspace}
% EOF: def_panda_sym.tex

